The Weights can be Harmful: Pareto Search versus Weighted Search in Multi-Objective Search-Based Software Engineering

In presence of multiple objectives to be optimized in Search-Based Software Engineering (SBSE), Pareto search has been commonly adopted. It searches for a good approximation of the problem's Pareto optimal solutions, from which the stakeholders choose the most preferred solution according to their preferences. However, when clear preferences of the stakeholders (e.g., a set of weights which reflect relative importance between objectives) are available prior to the search, weighted search is believed to be the first choice since it simplifies the search via converting the original multi-objective problem into a single-objective one and enable the search to focus on what only the stakeholders are interested in. This paper questions such a "weighted search first" belief. We show that the weights can, in fact, be harmful to the search process even in the presence of clear preferences. Specifically, we conduct a large scale empirical study which consists of 38 systems/projects from three representative SBSE problems, together with two types of search budget and nine sets of weights, leading to 604 cases of comparisons. Our key finding is that weighted search reaches a certain level of solution quality by consuming relatively less resources at the early stage of the search; however, Pareto search is at the majority of the time (up to 77% of the cases) significantly better than its weighted counterpart, as long as we allow a sufficient, but not unrealistic search budget. This, together with other findings and actionable suggestions in the paper, allows us to codify pragmatic and comprehensive guidance on choosing weighted and Pareto search for SBSE under the circumstance that clear preferences are available. All code and data can be accessed at: https://github.com/ideas-labo/pareto-vs-weight-for-sbse.

==> tables/new/normalization-3o-bk.tex <==


\begin{table*}[t!]
\caption{Scott-Knott ranks and the weighted scores for the normalization methods on three objectives SBSE problems. A cell summarizes 32 cases (4 algorithms $\times$ 4 weight vectors $\times$ 2 types of budget) on 100 runs each. Formats are the same as Table~\ref{tb:rq1}.}
    \label{tb:rq1-3}
    \footnotesize
    \setlength{\tabcolsep}{1.5mm}
  \begin{center}
    %\begin{adjustbox}{max width = 1\textwidth}
     

    \begin{tabular}{cc@{}cc@{}cc@{}cc}
        \begin{tabular}{llcc}
            \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline




\texttt{Dynamic}&&64&  \quart{13.151313341998401}{37.39710328768571}{15.575176437843362}{100}\\ 
\texttt{Fixed} &&\cellcolor{steel!10}\textbf{40}&  \bquart{11.533037255630886}{2.530153737830307}{11.454471491832251}{100}\\ 
\texttt{Ratio}&&54&  \quart{9.219464874187485}{23.690197016746236}{11.595156539237436}{100}\\ 
\texttt{None}&&82&  \quart{14.692677206958171}{85.30732279304183}{46.25035534856221}{100}\\ &&& \squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                     \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&\cellcolor{steel!10}\textbf{32}&  \bquart{14.179700338569672}{47.72674865630259}{27.573807004559747}{100}\\ 
&\cellcolor{steel!10}\textbf{32}&  \quart{14.112001914222759}{61.825460361051555}{28.053165682660957}{100}\\ 
&34&  \quart{16.227685355263443}{51.32318226742122}{28.97821654064092}{100}\\ 
&36&  \quart{16.47716348777977}{83.52283651222022}{27.25628401050523}{100}\\ && \squart{1}{1}{1}{100}\\ 

        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&44&  \quart{10.664724113022277}{15.602171008559319}{16.67328104378922}{100}\\ 
&82&  \quart{15.673756751940374}{42.702341361264516}{41.24999999999999}{100}\\ 
&91&  \quart{15.752810173731774}{84.24718982626823}{41.24999999999999}{100}\\ 
&\cellcolor{steel!10}\textbf{41}&  \bquart{10.698037623133938}{20.296696543498808}{13.650197175595753}{100}\\ && \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&51&  \quart{9.955924086289214}{48.108415402874925}{21.833878378343094}{100}\\ 
&83&  \quart{22.93050313527677}{64.59201605457427}{32.8545494847544}{100}\\ 
&102&  \quart{26.431295426942267}{73.56870457305773}{32.9989064078404}{100}\\ 
&\cellcolor{steel!10}\textbf{32}&  \bquart{6.783444043988988}{29.3853420780792}{16.369733318630466}{100}\\ && \squart{1}{1}{1}{100}\\ 

        \end{tabular} 
        \\
        
      
               (a). SCT: \textsc{vp8}&& (b). SCT: \textsc{hsqldb} && (c). WSC: \textsc{5as-3o}&& (d). WSC: \textsc{10as-3o}

\\
        \\
        
             \begin{tabular}{llcc}
              \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline


\texttt{Dynamic}&&56&  \quart{22.072088843370306}{55.5476934566427}{29.76751514929751}{100}\\ 
\texttt{Fixed} &&67&  \quart{22.072088843370306}{71.17292171650848}{31.370005941238475}{100}\\ 
\texttt{Ratio}&&77&  \quart{22.072088843370306}{77.92791115662969}{33.0826284826744}{100}\\ 
\texttt{None}&&\cellcolor{steel!10}\textbf{42}&  \bquart{15.637473371231442}{29.80707757528578}{25.041165156631305}{100}\\ 
&&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
        \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&50&  \quart{34.230449438489075}{34.36810854502177}{47.724400764709245}{100}\\ 
&\cellcolor{steel!10}\textbf{32}&  \bquart{28.51159792858015}{32.65416181973084}{34.48499707023807}{100}\\ 
&48&  \quart{35.51406643853247}{35.726056379557}{53.52957319438615}{100}\\ 
&74&  \quart{41.34571526324316}{58.65428473675684}{73.39059961629725}{100}\\  
&& \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
        \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&60&  \quart{44.64757011865832}{32.36160646304985}{62.30013448037588}{100}\\ 
&\cellcolor{steel!10}\textbf{34}&  \bquart{27.174591389206746}{40.58003744835758}{36.38901564132472}{100}\\ 
&48&  \quart{35.91467009943964}{37.80828483508155}{42.824133574134194}{100}\\ 
&66&  \quart{38.64632221690493}{61.353677783095065}{68.39896196974568}{100}\\ 
&& \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
        \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline

&51&  \quart{35.990913425070104}{45.98884395417154}{54.349046575171016}{100}\\ 
&\cellcolor{steel!10}\textbf{33}&  \bquart{28.555501356345225}{45.92741292105431}{33.49747965369362}{100}\\ 
&41&  \quart{28.67710700072914}{56.2420984606625}{41.209119987014596}{100}\\ 
&65&  \quart{38.70073994099188}{61.29926005900812}{70.56058204739927}{100}\\ 

&& \squart{1}{1}{1}{100}\\ 
        \end{tabular} 
        \\
        
      
               (e). WSC: \textsc{15as-3o}&& (f). NRP: \textsc{nrp-e-3o} && (g). NRP: \textsc{nrp-g-3o}&& (h). NRP: \textsc{nrp-m-3o}


        \\
    
    
    \end{tabular}
  %\end{adjustbox}
   \end{center}
\end{table*}




==> tables/new/normalization-bk.tex <==


\begin{table*}[t!]
\caption{\mytag{R2C3} \rev{Scott-Knott ranks and the weighted scores for the normalization methods on two objectives SBSE problems. A cell summarizes 72 cases (4 algorithms $\times$ 9 weight vectors $\times$ 2 types of budget) on 100 runs each. $\mathbfcal{R}$ denotes the total rank over all cases, hence a 72 means that a method has been ranked the first under each case. \quartexp{0}{20}{10}{20} denotes the 25th, 50th, and 75th percentile of the weighted score. \bquartexp{0}{20}{10}{20} denotes the best median among others. The best rank for each system has been highlighted.}}
%\caption{Comparing MOO$+$ with the other state-of-the-arts over 50 runs. SO$_{best}$ and MMO$_{best}$ denote the best single-objective optimizer and the MMO model with the best weight, respectively. \quartexp{0}{20}{10}{20} shows the average and standard deviation on the target performance objective achieved (all objective values are normalized and the closer to the left, the better). \bquartexp{0}{20}{10}{20} denote the best average among others. Column ``$\hat{A}_{12}$ ($p$ value)'' shows the $\hat{A}_{12}$ and $p$ value when comparing the corresponding counterpart with MOO$+$. The \setlength{\fboxsep}{1.5pt}\colorbox{steel!30}{blue cells} denote MMO$+$ wins while \setlength{\fboxsep}{1.5pt}\colorbox{red!10}{red cells} mean it loses; otherwise it is a tie. The statistically significant comparisons, i.e., $\hat{A}_{12} \geq 0.56$ (or $\hat{A}_{12} \leq 0.44$) and $p<0.05$ are highlighted in bold.}
    \label{tb:rq1}
    \footnotesize
    \setlength{\tabcolsep}{0.9mm}
  \begin{center}
    %\begin{adjustbox}{max width = 1\textwidth}
     

    \begin{tabular}{cc@{}cc@{}cc@{}cc@{}cc}
        \begin{tabular}{llcc}
            \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline

\texttt{Dynamic}&&114&  \bquart{0.3979324413585736}{0.6514456107368011}{0.6963817723775038}{100}\\ 
\texttt{Fixed} &&110&  \bquart{0.3979324413585736}{0.6019288580631452}{0.6963817723775038}{100}\\ 
\texttt{Ratio}&&114&  \quart{0.4602793748627034}{99.53972062513729}{0.805488906009731}{100}\\ 
\texttt{None}&&\cellcolor{steel!10}\textbf{104}&  \bquart{0.3979324413585736}{0.497415551698217}{0.6963817723775038}{100}\\ &&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                     \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&112&  \bquart{0.013597318031187121}{0.04344987355175401}{0.03434656230497302}{100}\\ 
&114&  \bquart{0.013597318031187121}{0.04406878524071667}{0.0344986008156132}{100}\\ 
&126&  \quart{0.02123161771681656}{99.97876838228316}{50.09476152618701}{100}\\ 
&\cellcolor{steel!10}\textbf{98}&  \bquart{0.013597318031187121}{0.04067656966037935}{0.03335523940535438}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&\cellcolor{steel!10}\textbf{72}&  \bquart{10.808388274864278}{9.999744852035786}{15.487061243289936}{100}\\ 
&76&  \quart{10.808388274864278}{10.078475148326413}{15.296013384311921}{100}\\ 
&148&  \quart{42.661419908381326}{57.33858009161868}{71.34709394142853}{100}\\ 
&74&  \quart{10.808388274864278}{9.999744852035786}{15.487061243289936}{100}\\ &&  \squart{1}{1}{1}{100}\\ 

        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&\cellcolor{steel!10}\textbf{72}&  \bquart{100}{0.0}{100}{100}\\ 
&\cellcolor{steel!10}\textbf{72}&  \bquart{100}{0.0}{100}{100}\\ 
&\cellcolor{steel!10}\textbf{72}&  \bquart{100}{0.0}{100}{100}\\ 
&\cellcolor{steel!10}\textbf{72}&  \bquart{100}{0.0}{100}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}&
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&\cellcolor{steel!10}\textbf{106}&  \bquart{42.807097615683055}{56.11206813959185}{67.68156239148234}{100}\\ 
&\cellcolor{steel!10}\textbf{106}&  \quart{42.807097615683055}{56.11206813959185}{68.17615624030596}{100}\\ 
&116&  \quart{42.807097615683055}{57.192902384316945}{71.34589645496871}{100}\\ 
&118&  \quart{42.807097615683055}{56.11206813959185}{70.41501145082432}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}  \\
               (a). SCT: \textsc{wc-c1-3d}&& (b). SCT: \textsc{wc-c3-3d} && (c). SCT: \textsc{wc-c4-3d}&& (d). SCT: \textsc{wc-c5-5d}&& (e). SCT: \textsc{rs-cd-6d}

\\
        \\
      
\begin{tabular}{llcc}
             \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline

\texttt{Dynamic}&&118&  \quart{43.50199071115998}{56.49800928884002}{73.98349256648626}{100}\\ 
\texttt{Fixed}&&120&  \quart{43.50199071115998}{54.37748838894998}{73.98349256648626}{100}\\ 
\texttt{Ratio}&&\cellcolor{steel!10}\textbf{98}&  \bquart{32.512288091703866}{43.6161956528261}{54.37748838894998}{100}\\ 
\texttt{None}&&110&  \quart{32.62649303336999}{57.98587646928916}{65.25298606673998}{100}\\ &&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&106&  \quart{23.127656689874083}{2.8614493863195856}{23.562297134563092}{100}\\ 
&\cellcolor{steel!10}\textbf{78}&  \bquart{21.53477256475079}{2.3305766229899616}{23.422733689020745}{100}\\ 
&172&  \quart{41.098643443309335}{58.901356556690665}{68.49773907218223}{100}\\ 
&110&  \quart{23.127656689874083}{3.9750327641803045}{23.68272045043106}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&\cellcolor{steel!10}\textbf{94}&  \bquart{25.331949151689546}{49.562360359529215}{50.08788831180633}{100}\\ 
&112&  \quart{36.201563679104375}{63.798436320895625}{65.60430644374968}{100}\\ 
&112&  \quart{38.149390750575016}{50.01290974151395}{63.2499197926609}{100}\\ 
&96&  \quart{25.232286197739857}{49.62157945397659}{50.02745038726599}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                   \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&150&  \quart{26.01611853293437}{34.3009351105759}{36.63557596651118}{100}\\ 
&149&  \quart{25.946873495192964}{35.618688324465175}{36.8487227716814}{100}\\ 
&175&  \quart{32.986164767955586}{67.01383523204441}{65.97232953591117}{100}\\ 
&\cellcolor{steel!10}\textbf{74}&  \bquart{12.550622907893262}{12.650043193642967}{16.79456349888235}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}&
        &
       \begin{tabular}{lcccl}
                     \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&\cellcolor{steel!10}\textbf{85}&  \bquart{23.61734906639778}{29.64113059235814}{40.91451626919466}{100}\\ 
&88&  \quart{23.61734906639778}{30.689464670899827}{40.90098835614948}{100}\\ 
&182&  \quart{43.64737843576848}{56.352621564231534}{69.8811705279697}{100}\\ 
&137&  \quart{34.24793619129034}{29.138998924167925}{52.235491992925}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}  \\
            (f). SCT: \textsc{wc-c1-6d}&& (g). SCT: \textsc{llvm} && (h). SCT: \textsc{trimesh}&& (i). WSC: \textsc{5as-1} && (j). WSC: \textsc{5as-2}
            
            \\
            \\
            
            
            
                  
\begin{tabular}{llcc}
             \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline


\texttt{Dynamic}&&101&  \quart{12.204269767327043}{15.935334789947499}{19.542343238155276}{100}\\ 
\texttt{Fixed}&&111&  \quart{14.464023232865971}{14.25283589617112}{19.944289851394625}{100}\\ 
\texttt{Ratio}&&198&  \quart{35.69980415105342}{64.30019584894657}{69.37212135322311}{100}\\ 
\texttt{None}&&\cellcolor{steel!10}\textbf{94}&  \bquart{11.073746598134948}{13.278867562036837}{17.360333405047168}{100}\\ &&&  \squart{1}{1}{1}{100}\\ 

        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                  \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\  
            \hline
&132&  \quart{26.297245639039687}{31.79725663200273}{40.8970604213949}{100}\\ 
&132&  \quart{26.25268519091374}{32.17859752520973}{41.1163900178106}{100}\\ 
&173&  \quart{29.427029732320936}{70.57297026767907}{53.5055221911625}{100}\\ 
&\cellcolor{steel!10}\textbf{73}&  \bquart{8.88095347535758}{32.03102081085784}{18.590442398073925}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&112&  \quart{9.28706562957637}{41.65881830834373}{30.58165928178645}{100}\\ 
&134&  \quart{11.055699844027641}{40.23335144136241}{31.102905084901224}{100}\\ 
&210&  \quart{33.42509800947557}{66.57490199052442}{59.360851432081866}{100}\\ 
&\cellcolor{steel!10}\textbf{76}&  \bquart{9.226120201993037}{29.26099071320306}{19.487917014297217}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                   \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&109&  \quart{4.752424900709067}{49.89404150244919}{30.44360030384378}{100}\\ 
&122&  \quart{6.132496355723156}{48.65586342316889}{30.458339616397918}{100}\\ 
&196&  \quart{29.700259887302693}{70.29974011269732}{53.60242272932956}{100}\\ 
&\cellcolor{steel!10}\textbf{79}&  \bquart{5.164537268775453}{34.64885420266566}{12.790319647738475}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}&
        &
       \begin{tabular}{lcccl}
                     \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&121&  \quart{23.39781512804246}{43.14746740256462}{39.90989709678373}{100}\\ 
&123&  \quart{23.85701908002895}{42.558397686779244}{40.24956297327387}{100}\\ 
&167&  \quart{24.113660912743658}{75.88633908725635}{52.698181099744914}{100}\\ 
&\cellcolor{steel!10}\textbf{75}&  \bquart{6.644177731633728}{39.75954988829815}{22.01921039827933}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}  \\
         (k). WSC: \textsc{5as-3}&& (l). WSC: \textsc{10as-1} && (m). WSC: \textsc{10as-2}&& (n). WSC: \textsc{10as-3} && (o). WSC: \textsc{15as-1}
            
            \\
            \\
            
            
                              
\begin{tabular}{llcc}
             \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline



\texttt{Dynamic}&&103&  \quart{13.834840784365333}{58.95418958880123}{42.720463221041804}{100}\\ 
\texttt{Fixed}&&135&  \quart{15.441904219170985}{59.426932759076934}{45.35997910482928}{100}\\ 
\texttt{Ratio}&&194&  \quart{23.162856328756476}{76.83714367124352}{53.08473230325475}{100}\\ 
\texttt{None}&&\cellcolor{steel!10}\textbf{75}&  \bquart{3.2417689847629267}{50.80616770706335}{22.088079532770717}{100}\\ &&&  \squart{1}{1}{1}{100}\\ 

        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&\cellcolor{steel!10}\textbf{96}&  \bquart{16.445541981942707}{58.03134462925001}{44.43830539732299}{100}\\ 
&117&  \quart{18.208089709372736}{57.89308553449767}{45.608789734334735}{100}\\ 
&169&  \quart{24.668312972914062}{75.33168702708593}{52.52084895737018}{100}\\ 
&105&  \quart{17.73627185448751}{39.398273766163}{30.64280088398862}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
     \end{tabular} &
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&136&  \quart{8.330621655580229}{79.2132432830263}{29.26321895555792}{100}\\ 
&122&  \quart{7.943545034298062}{80.28064625886825}{28.400949529640528}{100}\\ 
&170&  \quart{8.609015119541178}{91.39098488045883}{32.866989736115904}{100}\\ 
&\cellcolor{steel!10}\textbf{72}&  \bquart{5.344576122527188}{30.507169989590576}{18.71350916295027}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                   \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&151&  \quart{22.341217742647995}{20.235726924698525}{31.06127211722936}{100}\\ 
&\cellcolor{steel!10}\textbf{86}&  \bquart{11.636561121378062}{23.11763268168239}{14.044122341907284}{100}\\ 
&175&  \quart{33.082285076928464}{28.28525592835359}{41.326423695515125}{100}\\ 
&144&  \quart{24.41775385057225}{75.58224614942775}{42.90526519183438}{100}\\ &&  \squart{1}{1}{1}{100}\\ 

        \end{tabular}&
        &
       \begin{tabular}{lcccl}
                     \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&147&  \quart{19.123694795056675}{17.600254307089774}{27.071040424350283}{100}\\ 
&\cellcolor{steel!10}\textbf{85}&  \bquart{12.79948748428287}{17.523504640342843}{15.647465737068}{100}\\ 
&178&  \quart{29.658810093240973}{23.122780425897233}{37.03855021501507}{100}\\ 
&154&  \quart{22.80973001467084}{77.19026998532917}{38.9582850579088}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}  \\
        (p). WSC: \textsc{15as-2}&& (q). WSC: \textsc{15as-3} && (r). WSC: \textsc{50as}&& (s). NRP: \textsc{nrp-e1} && (t). NRP: \textsc{nrp-e2}

\\
\\


\begin{tabular}{llcc}
             \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline


\texttt{Dynamic}&&\cellcolor{steel!10}\textbf{74}&  \bquart{16.661095542392882}{9.014098719767409}{21.670302924289913}{100}\\ 
\texttt{Fixed}&&137&  \quart{22.94858065671771}{7.427532185454152}{28.07368456276078}{100}\\ 
\texttt{Ratio}&&138&  \quart{23.243282331608228}{33.899574811248925}{27.539353956018537}{100}\\ 
\texttt{None}&&197&  \quart{28.94619104637752}{71.05380895362248}{42.85714285714286}{100}\\ &&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&152&  \quart{18.92102425079402}{16.67900002567233}{27.052084780470203}{100}\\ 
&\cellcolor{steel!10}\textbf{86}&  \bquart{10.719298797910277}{17.358559781562555}{12.283311085559241}{100}\\ 
&184&  \quart{27.62909925382001}{21.04246187549099}{34.05184693771115}{100}\\ 
&154&  \quart{21.845805483165798}{78.1541945168342}{36.27165317407346}{100}\\ &&  \squart{1}{1}{1}{100}\\ 

     \end{tabular} &
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&141&  \quart{23.13425097294004}{11.218181940760687}{30.3761694292825}{100}\\ 
&\cellcolor{steel!10}\textbf{78}&  \bquart{16.021865725092532}{8.962350547147993}{19.440598138500718}{100}\\ 
&170&  \quart{28.252601924787655}{21.747398075212345}{38.89481442175938}{100}\\ 
&171&  \quart{23.504504273602606}{76.4954957263974}{35.052993351947585}{100}\\ &&  \squart{1}{1}{1}{100}\\ 

        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                   \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&146&  \quart{21.080813687889062}{14.916507614923088}{28.806928464112442}{100}\\ 
&\cellcolor{steel!10}\textbf{85}&  \bquart{11.234147667245937}{14.823429654733895}{13.868494272865213}{100}\\ 
&192&  \quart{32.71247858273002}{12.2880337245305}{38.487544746447945}{100}\\ 
&154&  \quart{18.8815548657838}{81.11844513421619}{34.63831427616412}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}&
        &
       \begin{tabular}{lcccl}
                     \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&152&  \quart{18.52438759333811}{15.22070012958911}{25.36521823816693}{100}\\ 
&\cellcolor{steel!10}\textbf{86}&  \bquart{10.182761563475088}{16.092549925933625}{11.64879421774698}{100}\\ 
&176&  \quart{26.227242612521298}{24.290461831666562}{33.333333333333336}{100}\\ 
&149&  \quart{19.92286302043245}{80.07713697956756}{33.333333333333336}{100}\\ &&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}  \\
      (u). NRP: \textsc{nep-e3}&& (v). NRP: \textsc{nrp-e4} && (w). NRP: \textsc{nrp-g1}&& (x). NRP: \textsc{nrp-g2} && (y). NRP: \textsc{nrp-g3}
     
     \\
     \\
     
     
     \begin{tabular}{llcc}
             \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline

 \texttt{Dynamic}&&147&  \quart{20.38628759248404}{16.737036231041284}{27.850594655876197}{100}\\ 
\texttt{Fixed}&&\cellcolor{steel!10}\textbf{86}&  \bquart{9.142848910467762}{20.083221827043797}{11.330138195582578}{100}\\ 
\texttt{Ratio}&&184&  \quart{32.05554766205612}{18.594139317961485}{39.55968623669914}{100}\\ 
\texttt{None}&&152&  \quart{22.03300938881011}{77.96699061118989}{36.84313798419947}{100}\\ &&&  \squart{1}{1}{1}{100}\\ 

        \end{tabular} & 
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline

&\cellcolor{steel!10}\textbf{110}&  \bquart{15.262430366081844}{14.16652668830501}{21.09919757149688}{100}\\ 
&115&  \quart{15.81517860601018}{10.35041274963856}{22.214644688247738}{100}\\ 
&156&  \quart{22.917932351617807}{37.13821897450535}{32.680086113050784}{100}\\ 
&155&  \quart{21.691513231255197}{78.30848676874481}{33.0990871015136}{100}\\ 
&&  \squart{1}{1}{1}{100}\\ 
     \end{tabular} &
        &
       \begin{tabular}{lcccl}
                    \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline

&139&  \quart{16.46965052841375}{14.550377359606681}{23.03609394897478}{100}\\ 
&\cellcolor{steel!10}\textbf{85}&  \bquart{12.043890863061208}{12.731357812862559}{13.84548118039925}{100}\\ 
&184&  \quart{25.712702131983992}{19.845751786298244}{31.75632951779306}{100}\\ 
&159&  \quart{19.86379316275183}{80.13620683724817}{33.333333333333336}{100}\\ 
&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcccl}
                   \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&\cellcolor{steel!10}\textbf{80}&  \bquart{16.604354996254276}{10.431678162002074}{21.95457812955959}{100}\\ 
&140&  \quart{22.605242323179873}{10.315242018943053}{28.021504466005258}{100}\\ 
&138&  \quart{20.922524512315928}{36.22033263054122}{28.17346177805487}{100}\\ 
&189&  \quart{28.400663523082446}{71.59933647691756}{37.66232406219442}{100}\\ 
&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}&
        &
       \begin{tabular}{lcccl}
                     \cellcolor[gray]{1}\textbf{}  &\cellcolor[gray]{1}$\mathbfcal{R}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&128&  \quart{15.716742075780354}{14.859656368864012}{22.386195961722354}{100}\\ 
&\cellcolor{steel!10}\textbf{93}&  \bquart{14.297150334823497}{11.774985429024944}{18.020033018078305}{100}\\ 
&162&  \quart{20.023063132584028}{37.11979401027312}{32.15422587390674}{100}\\ 
&150&  \quart{21.111694376261582}{78.88830562373842}{33.714400743651375}{100}\\ 
&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}  \\
       (z). NRP: \textsc{nep-g4}&& (aa). NRP: \textsc{nrp-m1} && (bb). NRP: \textsc{nrp-m2}&& (cc). NRP: \textsc{nrp-m3} && (dd). NRP: \textsc{nrp-m4}
     
    \end{tabular}
  %\end{adjustbox}
   \end{center}
\end{table*}




==> tables/new/quality-3o-bk.tex <==


\begin{table*}[t!]
\caption{\mytag{R2C8, R2C9} \rev{Pairwise comparisons (by $\hat{A}_{12}$ and Wilcoxon rank-sum test) and the weighted scores for Pareto and weighted search on three objectives SBSE problems. A pair summarizes 8 cases (4 weight vectors $\times$ 2 types of budget) on 100 runs each. Formats are the same as Table~\ref{tb:rq2}.}}
    \label{tb:rq2-3}
    \footnotesize
    \setlength{\tabcolsep}{0.5mm}
  \begin{center}
    \begin{adjustbox}{max width = \textwidth}
     

    \begin{tabular}{cc@{}cc@{}cc@{}cc}
        \begin{tabular}{llP{0.73cm}P{0.73cm}P{0.5cm}c}
            \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$ 
              &\cellcolor[gray]{1}$\mathbfcal{T}$& \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline


W$_{best}$&&-&-&-&   \quart{82.09324913931685}{17.906750860683154}{89.6895005146039}{100}\\ 
NSGA-II&&\cellcolor{steel!10}\textbf{3(3)}&\cellcolor{steel!10}1(0)&\cellcolor{steel!10}4&   \quart{78.08216789712984}{13.047185490541567}{82.8814483774804}{100}\\ 
MOEA/D&&\cellcolor{steel!10}3(1)&\cellcolor{steel!10}1(1)&\cellcolor{steel!10}4&   \quart{80.65620030713468}{19.343799692865314}{85.34382116580915}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular} & 
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.5cm}cl}
                        \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$   &\cellcolor[gray]{1}$\mathbfcal{T}$& \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{2.5675933222224776}{9.15912241056222}{4.832644983207379}{100}\\ 
&&\cellcolor{red!10}1(0)&\cellcolor{red!10}3(0)&\cellcolor{red!10}4&   \quart{3.0395962393806553}{6.836595037137648}{5.615653332963094}{100}\\ 
&&\cellcolor{red!10}0(0)&\cellcolor{red!10}4(0)&\cellcolor{red!10}4&   \quart{3.0941623147136466}{96.90583768528634}{7.632894392167036}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.5cm}cl}
                      \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$ &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{71.76757061725999}{28.232429382740005}{73.5156520836543}{100}\\ 
&&\cellcolor{steel!10}\textbf{6(6)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}2&  \quart{54.40586285203558}{32.651600592978035}{73.5156520836543}{100}\\ 
&&\cellcolor{steel!10}\textbf{6(6)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}2&  \quart{54.40586285203558}{32.651600592978035}{73.5156520836543}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 




        \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.5cm}cl}
                        \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$ &\cellcolor[gray]{1}$\mathbfcal{T}$  & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{89.99617664244441}{10.003823357555593}{92.5263191337284}{100}\\ 
&&\cellcolor{steel!10}\textbf{8(8)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}0&  \quart{61.183807145343515}{23.094596617393506}{83.70041770907655}{100}\\ 
&&\cellcolor{steel!10}\textbf{8(8)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}0&   \quart{61.183807145343515}{23.094596617393506}{83.70041770907655}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular}
         \\
         (a). SCT: \textsc{vp8}&& (b). SCT: \textsc{hsqldb} && (c). WSC: \textsc{5as-3o}&& (d). WSC: \textsc{10as-3o}


\\
        \\
      
 

           \begin{tabular}{llP{0.73cm}P{0.73cm}P{0.5cm}c}
                \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$ 
              &\cellcolor[gray]{1}$\mathbfcal{T}$& \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline



W$_{best}$&&-&-&-&   \quart{30.3030303030303}{69.69696969696969}{41.98627090112049}{100}\\ 
NSGA-II&&\textbf{4(2)}&4(0)&0&  \quart{30.3030303030303}{29.992024794470918}{41.98627090112049}{100}\\ 
MOEA/D&&\cellcolor{red!10}\textbf{3(2)}&\cellcolor{red!10}5(0)&\cellcolor{red!10}0&  \quart{30.3030303030303}{29.992024794470918}{41.98627090112049}{100}\\ 



&&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular} & 
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.5cm}cl}
            \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$ 
              &\cellcolor[gray]{1}$\mathbfcal{T}$& \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{59.893895493915096}{40.1061045060849}{80.65369894737574}{100}\\ 
&&\cellcolor{steel!10}\textbf{6(4)}&\cellcolor{steel!10}2(1)&\cellcolor{steel!10}0&  \quart{56.09254201264005}{42.13278829963255}{76.46235318482616}{100}\\ 
&&\cellcolor{steel!10}\textbf{8(7)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}0&  \quart{55.05835870051714}{41.038260847039496}{73.87109868546713}{100}\\ 




&&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.5cm}cl}
            \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$ 
              &\cellcolor[gray]{1}$\mathbfcal{T}$& \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{66.71658925058067}{23.746693200470034}{77.48988972764963}{100}\\ 
&&\cellcolor{red!10}2(2)&\cellcolor{red!10}\textbf{6(4)}&\cellcolor{red!10}0&   \quart{66.23113070218689}{27.528900440690194}{81.03100812076661}{100}\\ 
&&\cellcolor{steel!10}\textbf{5(5)}&\cellcolor{steel!10}3(1)&\cellcolor{steel!10}0&   \quart{66.71658925058067}{33.28341074941934}{75.97860766176464}{100}\\ 


&&&&&  \squart{1}{1}{1}{100}\\ 
      \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.5cm}cl}
            \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$ 
              &\cellcolor[gray]{1}$\mathbfcal{T}$& \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{69.13270882852346}{30.86729117147655}{85.83673398478174}{100}\\ 
&&\textbf{4(4)}&4(3)& 0& \quart{58.482241001603526}{34.96558882306159}{85.25763560029297}{100}\\ 
&&\cellcolor{steel!10}\textbf{7(7)}&\cellcolor{steel!10}1(0)&\cellcolor{steel!10}0&  \quart{53.833061416914674}{31.456815783592358}{70.82407171146555}{100}\\ 



&&&&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}
        
        
        \\
        
         
              (e). WSC: \textsc{15as-3o}&& (f). NRP: \textsc{nrp-e-3o} && (g). NRP: \textsc{nrp-g-3o}&& (h). NRP: \textsc{nrp-m-3o}

     
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}




==> tables/new/quality-bk.tex <==


\begin{table*}[t!]
\caption{\mytag{R2C3, R2C9} \rev{Pairwise comparisons (by $\hat{A}_{12}$ and Wilcoxon rank-sum test) and the weighted scores for Pareto and weighted search on two objectives SBSE problems. \quartexp{0}{20}{10}{20} denotes the 25th, 50th, and 75th percentile of the weighted score. A pair summarizes 18 cases (9 weight vectors $\times$ 2 types of budget) on 100 runs each. $W_{best}$ represents the best single objective algorithm and the normalization for the weighted search. $\mathbfcal{W}$ and $\mathbfcal{L}$ show how many cases the Pareto search wins ($\hat{A}_{12} > 0.5$) and loses ($\hat{A}_{12} < 0.5$) to the weighted counterpart, respectively. $\mathbfcal{T}$ denotes tie ($\hat{A}_{12} = 0.5$). The comparisons where the Pareto search and its weighed counterpart wins more are shown in \setlength{\fboxsep}{1.5pt}\colorbox{steel!10}{blue} and \setlength{\fboxsep}{1.5pt}\colorbox{red!30}{red}, respectively. The number in the bracket shows how many win/lose is statistically significant, i.e., $\hat{A}_{12} \geq 0.56$ (or $\hat{A}_{12} \leq 0.44$) and $p<0.05$. The one that with more statistically significant wins is highlighted in bold.}
}

    \label{tb:rq2}
    \footnotesize
    \setlength{\tabcolsep}{0.2mm}
  \begin{center}
    \begin{adjustbox}{max width = \textwidth}
     

    \begin{tabular}{cc@{}cc@{}cc@{}cc@{}cc}
        \begin{tabular}{llP{0.73cm}P{0.73cm}P{0.5cm}c}
            \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
W$_{best}$&&-&-&-& \quart{33.333333333333336}{50.0}{57.833859095688744}{100}\\ 
NSGA-II&&\cellcolor{steel!10}\textbf{18(8)}& \cellcolor{steel!10}0(0)& \cellcolor{steel!10}0& \quart{33.333333333333336}{33.333333333333336}{50.0}{100}\\ 
MOEA/D&&\cellcolor{red!10}8(6)&\cellcolor{red!10}\textbf{10(10)}&\cellcolor{red!10}0&  \quart{38.555906063792506}{61.444093936207494}{66.66666666666667}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
                        \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$   &\cellcolor[gray]{1}$\mathbfcal{T}$& \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{20.208724982786794}{79.79127501721321}{53.71612473986747}{100}\\ 
&&\cellcolor{steel!10}\textbf{14(12)}&\cellcolor{steel!10}4(0)&\cellcolor{steel!10}0&  \quart{20.208724982786794}{36.52455110203389}{45.469631211270276}{100}\\ 
&&\cellcolor{steel!10}\textbf{12(10)}&\cellcolor{steel!10}6(6)&\cellcolor{steel!10}0&  \quart{35.36526871987688}{59.53677701188543}{50.85916436082383}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
                      \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$ &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{46.22682518063205}{37.74438349173427}{64.15121678708805}{100}\\ 
&&\cellcolor{red!10}4(4)&\cellcolor{red!10}\textbf{14(12)}&\cellcolor{red!10}0&  \quart{48.76796760192136}{41.908254867448605}{69.87690609791545}{100}\\ 
&&\cellcolor{red!10}6(4)&\cellcolor{red!10}\textbf{12(10)}&\cellcolor{red!10}0&  \quart{46.22682518063205}{53.77317481936795}{73.11341259031603}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
                        \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  &\cellcolor[gray]{1}$\mathbfcal{T}$& \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{90}{0.0}{90}{100}\\ 
&&0(0)&0(0)&18&  \quart{90}{0.0}{90}{100}\\ 
&&0(0)&0(0)&18&  \quart{90}{0.0}{90}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}&
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
                        \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
                   &\cellcolor[gray]{1}$\mathbfcal{T}$& \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{50.0}{50.0}{75.0}{100}\\ 
&&\cellcolor{steel!10}\textbf{12(12)}&\cellcolor{steel!10}6(4)&\cellcolor{steel!10}0&  \quart{49.77134677745473}{22.218616142221162}{61.8111587553415}{100}\\ &&\cellcolor{steel!10}\textbf{12(10)}&\cellcolor{steel!10}6(6)&\cellcolor{steel!10}0&  \quart{49.908841123893936}{27.35936444528037}{62.51017666406477}{100}\\&&&&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}  \\
            (a). SCT: \textsc{wc-c1-3d}&& (b). SCT: \textsc{wc-c3-3d} && (c). SCT: \textsc{wc-c4-3d}&& (d). SCT: \textsc{wc-c5-5d}&& (e). SCT: \textsc{rs-cd-6d}

\\
        \\
      
           \begin{tabular}{llP{0.73cm}P{0.73cm}P{0.3cm}c}
             \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
W$_{best}$&&-&-&-&  \quart{42.95897187408059}{57.04102812591941}{64.61434133532391}{100}\\ 
NSGA-II&&\cellcolor{steel!10}\textbf{18(16)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}0&  \quart{22.755834300672213}{28.6616900079341}{37.579302598024555}{100}\\ 
MOEA/D&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}2(2)&\cellcolor{steel!10}0&  \quart{29.704792530381063}{29.53694833650825}{42.95897187408059}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} & 
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{52.39776975718294}{4.9527172999055775}{56.27352815616875}{100}\\ 
&&\cellcolor{steel!10}\textbf{14(2)}&\cellcolor{steel!10}2(0)&\cellcolor{steel!10}2&  \quart{52.39776975718294}{4.9527172999055775}{56.27352815616875}{100}\\ 
&&\cellcolor{red!10}0(0)&\cellcolor{red!10}\textbf{18(16)}&\cellcolor{red!10}0&  \quart{59.692630108278024}{40.307369891721976}{69.95769783055844}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{49.89762518938587}{50.10237481061413}{74.98275694705997}{100}\\ 
&&\cellcolor{steel!10}\textbf{18(16)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}0&  \quart{49.89762518938587}{49.65526934558496}{74.74722490131572}{100}\\ 
&&\cellcolor{steel!10}\textbf{14(12)}&\cellcolor{steel!10}4(4)&\cellcolor{steel!10}0&  \quart{49.98850463137332}{49.9699833732188}{74.98275694705997}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{45.87417594342628}{14.025095969492924}{47.19119530490584}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}2&  \quart{39.436841680325216}{5.2665284477978}{43.53256431281975}{100}\\ 
&&\cellcolor{red!10}2(2)&\cellcolor{red!10}\textbf{10(10)}&\cellcolor{red!10}6&  \quart{47.19119530490584}{52.80880469509417}{82.39706510163529}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 

        \end{tabular}&
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{60.383845704381606}{39.61615429561839}{81.90444700884846}{100}\\ 
&&\cellcolor{steel!10}\textbf{12(12)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}6&  \quart{50.282519652897165}{32.515683563999396}{75.14125982644858}{100}\\ 
&&\cellcolor{steel!10}\textbf{12(12)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}6&  \quart{50.282519652897165}{32.515683563999396}{75.14125982644858}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 

        \end{tabular}  \\
            (f). SCT: \textsc{wc-c1-6d}&& (g). SCT: \textsc{llvm} && (h). SCT: \textsc{trimesh}&& (i). WSC: \textsc{5as-1} && (j). WSC: \textsc{5as-2}
            
            \\
            \\
            
             \begin{tabular}{llP{0.73cm}P{0.73cm}P{0.3cm}c}
             \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline

W$_{best}$&&-&-&-&  \quart{55.13688147309497}{44.86311852690504}{92.85782883802584}{100}\\ 
NSGA-II&&\cellcolor{steel!10}\textbf{10(10)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}8&  \quart{55.13688147309497}{39.806980934514904}{77.56844073654749}{100}\\ 
MOEA/D&&\cellcolor{steel!10}\textbf{10(10)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}8&  \quart{55.13688147309497}{39.806980934514904}{77.56844073654749}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 

        \end{tabular} & 
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{57.08462453963534}{17.452462547517086}{58.72348898167366}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}2&  \quart{49.07417417430485}{6.553530235411825}{54.170784279798006}{100}\\ 
&&\cellcolor{red!10}6(6)&\cellcolor{red!10}12(6)&\cellcolor{red!10}0&  \quart{52.78717077207993}{47.21282922792007}{74.53708708715243}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 

        \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{50.19506373291404}{49.80493626708596}{81.39235622494458}{100}\\ 
&&\cellcolor{steel!10}\textbf{12(10)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}6&  \quart{48.32894279510596}{34.891877324777845}{67.99080098303102}{100}\\ 
&&\cellcolor{steel!10}\textbf{12(10)}&\cellcolor{steel!10}6(0)&\cellcolor{steel!10}0&  \quart{48.32894279510596}{34.891877324777845}{67.99080098303102}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 
      \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{70.30757328998216}{29.692426710017838}{76.27244966476577}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}2&  \quart{61.18082747102267}{15.913133207451043}{71.2707587086454}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}2(0)&\cellcolor{steel!10}0&  \quart{61.18082747102267}{15.913133207451043}{71.2707587086454}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 

        \end{tabular}&
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{57.08462453963535}{17.45246254751708}{58.72348898167366}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}2(0)&\cellcolor{steel!10}0&  \quart{49.07417417430485}{7.281990300371171}{54.17078427979803}{100}\\ 
&&\cellcolor{steel!10}\textbf{10(10)}&\cellcolor{steel!10}8(6)&\cellcolor{steel!10}0&  \quart{52.78717077207993}{47.21282922792007}{74.53708708715243}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 

        \end{tabular}  \\
            (k). WSC: \textsc{5as-3}&& (l). WSC: \textsc{10as-1} && (m). WSC: \textsc{10as-2}&& (n). WSC: \textsc{10as-3} && (o). WSC: \textsc{15as-1}
            
            \\
            \\
            
                         \begin{tabular}{llP{0.73cm}P{0.73cm}P{0.3cm}c}
             \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline

W$_{best}$&&-&-&-&  \quart{43.222779352304634}{56.777220647695366}{71.61138967615233}{100}\\ 
NSGA-II&&\cellcolor{red!10}2(0)&\cellcolor{red!10}16(0)&\cellcolor{red!10}0&  \quart{43.222779352304634}{56.777220647695366}{71.61138967615233}{100}\\ 
MOEA/D&&\cellcolor{red!10}1(0)&\cellcolor{red!10}16(0)&\cellcolor{red!10}1&  \quart{43.222779352304634}{56.777220647695366}{71.61138967615233}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular} & 
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{55.56892085387591}{44.431079146124084}{83.35338128081386}{100}\\ 
&&\cellcolor{red!10}\textbf{7(6)}&\cellcolor{red!10}11(0)&\cellcolor{red!10}0&  \quart{55.56892085387591}{37.498055074002956}{83.35338128081386}{100}\\ 
&&\cellcolor{steel!10}\textbf{9(6)}&\cellcolor{steel!10}9(0)&\cellcolor{steel!10}0&  \quart{55.56892085387591}{37.45298387406728}{83.35338128081386}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{25.627697079745527}{74.37230292025447}{78.26050900694321}{100}\\ 
&&\cellcolor{steel!10}\textbf{11(10)}&\cellcolor{steel!10}7(6)&\cellcolor{steel!10}0&  \quart{48.41449065469265}{48.111889089820835}{72.12649627190042}{100}\\ 
&&\cellcolor{steel!10}\textbf{11(9)}&\cellcolor{steel!10}7(7)&\cellcolor{steel!10}0&  \quart{48.657126767303666}{47.364979977365934}{72.79203477897946}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 


      \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{79.16643067893632}{20.83356932106368}{94.05633881749344}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(15)}&\cellcolor{steel!10}2(2)&\cellcolor{steel!10}0&  \quart{64.3299822149323}{14.41985732498049}{73.44700878765691}{100}\\ 
&&\cellcolor{steel!10}\textbf{15(14)}&\cellcolor{steel!10}3(2)&\cellcolor{steel!10}0&  \quart{65.87284105545548}{13.63475759134282}{74.69112036960378}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular}&
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{72.0547041386723}{27.945295861327693}{95.1108584898767}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}2(2)&\cellcolor{steel!10}0&  \quart{59.686301057958}{12.334088251124454}{67.67661736466343}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}2(2)&\cellcolor{steel!10}0&  \quart{58.39393521191114}{12.69503499931395}{66.31731860601577}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular}  \\
            (p). WSC: \textsc{15as-2}&& (q). WSC: \textsc{15as-3} && (r). WSC: \textsc{50as}&& (s). NRP: \textsc{nrp-e1} && (t). NRP: \textsc{nrp-e2}
\\
\\


           \begin{tabular}{llP{0.73cm}P{0.73cm}P{0.3cm}c}
             \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline


W$_{best}$&&-&-&-&  \quart{66.58579428745222}{33.414205712547776}{86.5244018463966}{100}\\ 
NSGA-II&&\cellcolor{steel!10}\textbf{18(18)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}0&  \quart{64.10160808027831}{20.28544699316382}{77.14736559128052}{100}\\ 
MOEA/D&&\cellcolor{steel!10}\textbf{18(18)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}0&  \quart{64.10160808027831}{20.130165874151558}{77.14736559128052}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular} & 
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{81.41718776836423}{18.58281223163577}{92.9223799853293}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(14)}&\cellcolor{steel!10}2(2)&\cellcolor{steel!10}0&  \quart{66.15688103825599}{15.136998891148652}{76.42943771481127}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}2(2)&\cellcolor{steel!10}0&  \quart{65.20249168763532}{13.879623083663267}{75.30452102427502}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 



        \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{73.56061498238812}{26.439385017611883}{95.47718988040391}{100}\\ 
&&\cellcolor{steel!10}\textbf{18(18)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}0&  \quart{69.49795708724436}{20.1093970161112}{82.32952566653006}{100}\\ 
&&\cellcolor{steel!10}\textbf{18(18)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}0&  \quart{69.49795708724436}{19.888983354957855}{82.32952566653006}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 


      \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{79.21405162830634}{20.785948371693657}{89.15502257477853}{100}\\ 
&&\cellcolor{steel!10}\textbf{18(18)}&\cellcolor{steel!10}0(0)&-
\cellcolor{steel!10}0&  \quart{59.53802969496109}{15.905217016925493}{69.86834471980089}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}2(1)&\cellcolor{steel!10}0&  \quart{61.37662076341841}{14.066625948468166}{70.59061646362687}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 

        \end{tabular}&
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline

&&-&-&-&  \quart{82.32570224137227}{17.67429775862773}{95.14693531525178}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}2(2)&\cellcolor{steel!10}0&  \quart{69.8224644391288}{12.95809177393161}{78.6189911050402}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(15)}&\cellcolor{steel!10}2(2)&\cellcolor{steel!10}0&  \quart{69.93627515419045}{14.158720353794305}{79.68811007731095}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular}  \\
            (u). NRP: \textsc{nep-e3}&& (v). NRP: \textsc{nrp-e4} && (w). NRP: \textsc{nrp-g1}&& (x). NRP: \textsc{nrp-g2} && (y). NRP: \textsc{nrp-g3}
\\
\\

           \begin{tabular}{llP{0.73cm}P{0.73cm}P{0.3cm}c}
             \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
W$_{best}$&&-&-&-&  \quart{78.7458037261856}{21.254196273814397}{95.77982067843087}{100}\\ 
NSGA-II&&\cellcolor{steel!10}\textbf{12(12)}&\cellcolor{steel!10}6(6)&\cellcolor{steel!10}0&  \quart{76.79068737050768}{15.261313591579157}{85.9349363095412}{100}\\ 
MOEA/D&&\cellcolor{steel!10}\textbf{12(12)}&\cellcolor{steel!10}6(6)&\cellcolor{steel!10}0&  \quart{76.3443290497169}{12.862100516322485}{85.26674371666917}{100}\\ 

&&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular} & 
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{55.27077254884161}{44.72922745115839}{85.39756537587158}{100}\\ 
&&\cellcolor{steel!10}\textbf{17(16)}&\cellcolor{steel!10}1(0)&\cellcolor{steel!10}0&  \quart{40.83227248597352}{12.58941279291771}{48.59035765238844}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}2(2)&\cellcolor{steel!10}0&  \quart{42.22457322253468}{10.939791339188881}{48.839922916832904}{100}\\ 

&&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{77.06894514707989}{22.93105485292011}{89.83824019173825}{100}\\ 
&&\cellcolor{steel!10}\textbf{18(18)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}0&  \quart{56.11438061505086}{15.429166879707312}{65.53692406015314}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}2(2)&\cellcolor{steel!10}0&  \quart{56.88755139436752}{14.970661453366656}{66.62838946785793}{100}\\ 
&&&&&  \squart{1}{1}{1}{100}\\ 
      \end{tabular} &
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline
&&-&-&-&  \quart{62.8004728418531}{37.19952715814689}{89.13611986219446}{100}\\ 
&&\cellcolor{steel!10}\textbf{18(18)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}0&  \quart{59.827421323592645}{18.759865862896007}{70.95624696343025}{100}\\ 
&&\cellcolor{steel!10}\textbf{18(18)}&\cellcolor{steel!10}0(0)&\cellcolor{steel!10}0&  \quart{59.827421323592645}{18.713603461525896}{70.95624696343025}{100}\\ 
&&&&&  \squart{1}{1}{1}{100}\\ 
        \end{tabular}&
        &
       \begin{tabular}{lcP{0.73cm}P{0.73cm}P{0.3cm}cl}
         \cellcolor[gray]{1}\textbf{} & &\cellcolor[gray]{1}$\mathbfcal{W}$ &\cellcolor[gray]{1}$\mathbfcal{L}$  
            &\cellcolor[gray]{1}$\mathbfcal{T}$ & \cellcolor[gray]{1}\textbf{Quantiles}  \\
            \hline

&&-&-&-&  \quart{74.32146575636206}{25.67853424363793}{93.29990966511781}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}2(2)&\cellcolor{steel!10}0&  \quart{50.26853044990115}{11.063294685795789}{57.55431970466618}{100}\\ 
&&\cellcolor{steel!10}\textbf{16(16)}&\cellcolor{steel!10}2(2)&\cellcolor{steel!10}0&  \quart{49.81609346759535}{10.15972681719828}{56.55518039537364}{100}\\ &&&&&  \squart{1}{1}{1}{100}\\ 


        \end{tabular}  
        
        
        \\
        
         
            (z). NRP: \textsc{nep-g4}&& (aa). NRP: \textsc{nrp-m1} && (bb). NRP: \textsc{nrp-m2}&& (cc). NRP: \textsc{nrp-m3} && (dd). NRP: \textsc{nrp-m4}
     
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}




==> tables/normalization1.tex <==
\begin{table}[t!]%change two red to two green
\caption{Scott-Knott ranks of the fitness and the 25th, 50th, and 75th percentile of gains (\%) over \texttt{None} for the SCT problem. A cell summarizes 72 cases (4 algorithms $\times$ 9 weight vectors $\times$ 2 types of budget) on 100 runs each. The \textit{Rank} indicates the total rank over all cases, hence a 72 means that a method has been ranked the first under each case. The best rank for each system has been highlighted.}
\label{tb:norm1}
\centering
\footnotesize
\begin{tabular}{ccc|cc}\toprule

&\textbf{Rank}&\textbf{Gain Percentile}&\textbf{Rank}&\textbf{Gain Percentile}\\ \midrule


&\multicolumn{2}{c|}{\textsc{\textbf{wc-c1-3d}}}&\multicolumn{2}{c}{\textsc{\textbf{wc-c3-3d}}}\\  
\texttt{Dynamic}&114&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c1-3d-dynamic.pdf}}&112&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c3-3d-dynamic.pdf}}\\ 
\texttt{Fixed}&110&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c1-3d-fixed.pdf}}&114&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c3-3d-fixed.pdf}}\\ 
\texttt{Ratio}&114&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c1-3d-ratio.pdf}}&126&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c3-3d-ratio.pdf}}\\ 
\texttt{None}&\cellcolor{steel!10}\textbf{104}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c1-3d-none.pdf}}&\cellcolor{steel!10}\textbf{98}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c3-3d-none.pdf}}\\ \hline 


&\multicolumn{2}{c|}{\textsc{\textbf{wc-c4-3d}}}&\multicolumn{2}{c}{\textsc{\textbf{wc-c5-5d}}}\\  
\texttt{Dynamic}&\cellcolor{steel!10}\textbf{72}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c4-3d-dynamic.pdf}}&\cellcolor{steel!10}\textbf{72}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c5-5d-dynamic.pdf}}\\ 
\texttt{Fixed}&76&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c4-3d-fixed.pdf}}&\cellcolor{steel!10}\textbf{72}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c5-5d-fixed.pdf}}\\ 
\texttt{Ratio}&148&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c4-3d-ratio.pdf}}&\cellcolor{steel!10}\textbf{72}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c5-5d-ratio.pdf}}\\ 
\texttt{None}&74&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c4-3d-none.pdf}}&\cellcolor{steel!10}\textbf{72}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c5-5d-none.pdf}}\\ \hline 


&\multicolumn{2}{c|}{\textsc{\textbf{rs-c3-6d}}}&\multicolumn{2}{c}{\textsc{\textbf{wc-c1-6d}}}\\  
\texttt{Dynamic}&\cellcolor{steel!10}\textbf{106}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-rs-c3-6d-dynamic.pdf}}&118&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c1-6d-dynamic.pdf}}\\ 
\texttt{Fixed}&\cellcolor{steel!10}\textbf{106}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-rs-c3-6d-fixed.pdf}}&120&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c1-6d-fixed.pdf}}\\ 
\texttt{Ratio}&116&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-rs-c3-6d-ratio.pdf}}&\cellcolor{steel!10}\textbf{98}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c1-6d-ratio.pdf}}\\ 
\texttt{None}&118&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-rs-c3-6d-none.pdf}}&110&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-wc-c1-6d-none.pdf}}\\ \hline 


&\multicolumn{2}{c|}{\textsc{\textbf{llvm}}}&\multicolumn{2}{c}{\textsc{\textbf{trimesh}}}\\  
\texttt{Dynamic}&106&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-llvm-dynamic.pdf}}&\cellcolor{steel!10}\textbf{94}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-trimesh-dynamic.pdf}}\\ 
\texttt{Fixed}&\cellcolor{steel!10}\textbf{78}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-llvm-fixed.pdf}}&112&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-trimesh-fixed.pdf}}\\ 
\texttt{Ratio}&172&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-llvm-ratio.pdf}}&112&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-trimesh-ratio.pdf}}\\ 
\texttt{None}&110&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-llvm-none.pdf}}&96&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-trimesh-none.pdf}}\\  







%%%%

&&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/norm-error-bar-bottom-sct.pdf}}&&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/norm-error-bar-bottom-sct.pdf}}\\


\bottomrule
\end{tabular}



%}
\centering
% \begin{tablenotes}
   % \footnotesize
   % \item The $p$ values are shown in the bracket. $A_{12}>0.5$ means the Pareto search is better (highlighted in \colorbox{steel!10}{blue}); $A_{12}<0.5$ denotes the weighted search is better (highlighted in \colorbox{pink!120}{pink}); $A_{12}=0.5$ means a tie. In particular, $0.6\leq A_{12}<0.7$ or $0.3< A_{12}\leq0.4$ indicates a small effect size while $0.7 \leq A_{12} < 0.8$ or $0.2 < A_{12} \leq 0.3$ means a medium effect size; $A_{12} \geq 0.8$ or $0.2 \leq A_{12}$ indicates a large effect size. The comparisons, for which there is a statistically significant differences ($p<$.05) and non-trivial effect size ($A_{12} \leq 0.4$ or $A_{12} \geq 0.6$), are highlighted in \textbf{bold}.
    %\end{tablenotes}
\end{table}



==> tables/normalization2.tex <==
\begin{table}[t!]%change two red to two green

\caption{For the WSC problems. Same format as Table~\ref{tb:norm1}.}
\label{tb:norm2}
%\setlength{\tabcolsep}{1.2mm}
\centering
\footnotesize
\begin{tabular}{ccc|cc}\toprule

&\textbf{Rank}&\textbf{Gain Percentile}&\textbf{Rank}&\textbf{Gain Percentile}\\ \midrule


&\multicolumn{2}{c|}{\textsc{\textbf{5as-1}}}&\multicolumn{2}{c}{\textsc{\textbf{5as-2}}}\\  
\texttt{Dynamic}&150&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-5as-1-dynamic.pdf}}&\cellcolor{steel!10}\textbf{85}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-5as-2-dynamic.pdf}}\\ 
\texttt{Fixed}&149&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-5as-1-fixed.pdf}}&88&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-5as-2-fixed.pdf}}\\ 
\texttt{Ratio}&175&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-5as-1-ratio.pdf}}&182&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-5as-2-ratio.pdf}}\\ 
\texttt{None}&\cellcolor{steel!10}\textbf{74}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-5as-1-none.pdf}}&137&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-5as-2-none.pdf}}\\ \hline 


&\multicolumn{2}{c|}{\textsc{\textbf{5as-3}}}&\multicolumn{2}{c}{\textsc{\textbf{10as-1}}}\\  
\texttt{Dynamic}&101&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-5as-3-dynamic.pdf}}&132&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-10as-1-dynamic.pdf}}\\ 
\texttt{Fixed}&111&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-5as-3-fixed.pdf}}&132&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-10as-1-fixed.pdf}}\\ 
\texttt{Ratio}&198&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-5as-3-ratio.pdf}}&173&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-10as-1-ratio.pdf}}\\ 
\texttt{None}&\cellcolor{steel!10}\textbf{94}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-5as-3-none.pdf}}&\cellcolor{steel!10}\textbf{73}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-10as-1-none.pdf}}\\ \hline 


&\multicolumn{2}{c|}{\textsc{\textbf{10as-2}}}&\multicolumn{2}{c}{\textsc{\textbf{10as-3}}}\\  
\texttt{Dynamic}&112&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-10as-2-dynamic.pdf}}&109&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-10as-3-dynamic.pdf}}\\ 
\texttt{Fixed}&134&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-10as-2-fixed.pdf}}&122&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-10as-3-fixed.pdf}}\\ 
\texttt{Ratio}&210&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-10as-2-ratio.pdf}}&196&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-10as-3-ratio.pdf}}\\ 
\texttt{None}&\cellcolor{steel!10}\textbf{76}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-10as-2-none.pdf}}&\cellcolor{steel!10}\textbf{79}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-10as-3-none.pdf}}\\ \hline 


&\multicolumn{2}{c|}{\textsc{\textbf{15as-1}}}&\multicolumn{2}{c}{\textsc{\textbf{15as-2}}}\\  
\texttt{Dynamic}&121&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-15as-1-dynamic.pdf}}&103&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-15as-2-dynamic.pdf}}\\ 
\texttt{Fixed}&123&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-15as-1-fixed.pdf}}&135&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-15as-2-fixed.pdf}}\\ 
\texttt{Ratio}&167&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-15as-1-ratio.pdf}}&194&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-15as-2-ratio.pdf}}\\ 
\texttt{None}&\cellcolor{steel!10}\textbf{75}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-15as-1-none.pdf}}&\cellcolor{steel!10}\textbf{75}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-15as-2-none.pdf}}\\ \hline 


&\multicolumn{2}{c|}{\textsc{\textbf{15as-3}}}&\multicolumn{2}{c}{\textsc{\textbf{50as}}}\\  
\texttt{Dynamic}&\cellcolor{steel!10}\textbf{96}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-15as-3-dynamic.pdf}}&136&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-50as-dynamic.pdf}}\\ 
\texttt{Fixed}&117&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-15as-3-fixed.pdf}}&122&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-50as-fixed.pdf}}\\ 
\texttt{Ratio}&169&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-15as-3-ratio.pdf}}&170&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-50as-ratio.pdf}}\\ 
\texttt{None}&105&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-15as-3-none.pdf}}&\cellcolor{steel!10}\textbf{72}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-50as-none.pdf}}\\ 



&&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/norm-error-bar-bottom-service.pdf}}&&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/norm-error-bar-bottom-service.pdf}}\\


\bottomrule
\end{tabular}




%}
\centering
% \begin{tablenotes}
   % \footnotesize
   % \item The $p$ values are shown in the bracket. $A_{12}>0.5$ means the Pareto search is better (highlighted in \colorbox{steel!10}{blue}); $A_{12}<0.5$ denotes the weighted search is better (highlighted in \colorbox{pink!120}{pink}); $A_{12}=0.5$ means a tie. In particular, $0.6\leq A_{12}<0.7$ or $0.3< A_{12}\leq0.4$ indicates a small effect size while $0.7 \leq A_{12} < 0.8$ or $0.2 < A_{12} \leq 0.3$ means a medium effect size; $A_{12} \geq 0.8$ or $0.2 \leq A_{12}$ indicates a large effect size. The comparisons, for which there is a statistically significant differences ($p<$.05) and non-trivial effect size ($A_{12} \leq 0.4$ or $A_{12} \geq 0.6$), are highlighted in \textbf{bold}.
    %\end{tablenotes}
\end{table}

==> tables/normalization3.tex <==
\begin{table}[t!]%change two red to two green

\caption{For the NRP problems. Same format as Table~\ref{tb:norm1}.}
\label{tb:norm3}
%\setlength{\tabcolsep}{1.5mm}
\centering
\footnotesize
\begin{tabular}{ccc|cc}\toprule

&\textbf{Rank}&\textbf{Gain Percentile}&\textbf{Rank}&\textbf{Gain Percentile}\\ \midrule



&\multicolumn{2}{c|}{\textsc{\textbf{nrp-e1}}}&\multicolumn{2}{c}{\textsc{\textbf{nrp-e2}}}\\  
\texttt{Dynamic}&151&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e1-dynamic.pdf}}&147&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e2-dynamic.pdf}}\\ 
\texttt{Fixed}&\cellcolor{steel!10}\textbf{86}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e1-fixed.pdf}}&\cellcolor{steel!10}\textbf{85}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e2-fixed.pdf}}\\ 
\texttt{Ratio}&175&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e1-ratio.pdf}}&178&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e2-ratio.pdf}}\\ 
\texttt{None}&144&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e1-none.pdf}}&154&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e2-none.pdf}}\\ \hline 


&\multicolumn{2}{c|}{\textsc{\textbf{nrp-e3}}}&\multicolumn{2}{c}{\textsc{\textbf{nrp-e4}}}\\  
\texttt{Dynamic}&\cellcolor{steel!10}\textbf{74}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e3-dynamic.pdf}}&152&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e4-dynamic.pdf}}\\ 
\texttt{Fixed}&137&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e3-fixed.pdf}}&\cellcolor{steel!10}\textbf{86}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e4-fixed.pdf}}\\ 
\texttt{Ratio}&138&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e3-ratio.pdf}}&184&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e4-ratio.pdf}}\\ 
\texttt{None}&197&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e3-none.pdf}}&154&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-e4-none.pdf}}\\ \hline 


&\multicolumn{2}{c|}{\textsc{\textbf{nrp-g1}}}&\multicolumn{2}{c}{\textsc{\textbf{nrp-g2}}}\\  
\texttt{Dynamic}&141&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g1-dynamic.pdf}}&146&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g2-dynamic.pdf}}\\ 
\texttt{Fixed}&\cellcolor{steel!10}\textbf{78}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g1-fixed.pdf}}&\cellcolor{steel!10}\textbf{85}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g2-fixed.pdf}}\\ 
\texttt{Ratio}&170&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g1-ratio.pdf}}&192&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g2-ratio.pdf}}\\ 
\texttt{None}&171&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g1-none.pdf}}&154&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g2-none.pdf}}\\ \hline 


&\multicolumn{2}{c|}{\textsc{\textbf{nrp-g3}}}&\multicolumn{2}{c}{\textsc{\textbf{nrp-g4}}}\\  
\texttt{Dynamic}&152&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g3-dynamic.pdf}}&147&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g4-dynamic.pdf}}\\ 
\texttt{Fixed}&\cellcolor{steel!10}\textbf{86}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g3-fixed.pdf}}&\cellcolor{steel!10}\textbf{86}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g4-fixed.pdf}}\\ 
\texttt{Ratio}&176&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g3-ratio.pdf}}&184&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g4-ratio.pdf}}\\ 
\texttt{None}&149&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g3-none.pdf}}&152&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-g4-none.pdf}}\\ \hline 


&\multicolumn{2}{c|}{\textsc{\textbf{nrp-m1}}}&\multicolumn{2}{c}{\textsc{\textbf{nrp-m2}}}\\  
\texttt{Dynamic}&\cellcolor{steel!10}\textbf{110}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m1-dynamic.pdf}}&139&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m2-dynamic.pdf}}\\ 
\texttt{Fixed}&115&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m1-fixed.pdf}}&\cellcolor{steel!10}\textbf{85}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m2-fixed.pdf}}\\ 
\texttt{Ratio}&156&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m1-ratio.pdf}}&184&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m2-ratio.pdf}}\\ 
\texttt{None}&155&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m1-none.pdf}}&159&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m2-none.pdf}}\\ \hline 


&\multicolumn{2}{c|}{\textsc{\textbf{nrp-m3}}}&\multicolumn{2}{c}{\textsc{\textbf{nrp-m4}}}\\  
\texttt{Dynamic}&\cellcolor{steel!10}\textbf{80}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m3-dynamic.pdf}}&128&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m4-dynamic.pdf}}\\ 
\texttt{Fixed}&140&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m3-fixed.pdf}}&\cellcolor{steel!10}\textbf{93}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m4-fixed.pdf}}\\ 
\texttt{Ratio}&138&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m3-ratio.pdf}}&162&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m4-ratio.pdf}}\\ 
\texttt{None}&189&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m3-none.pdf}}&150&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/norm-error-bar-nrp-m4-none.pdf}}\\  








&&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/norm-error-bar-bottom-nrp.pdf}}&&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/norm-error-bar-bottom-nrp.pdf}}\\

\bottomrule
\end{tabular}




%}
\centering
% \begin{tablenotes}
   % \footnotesize
   % \item The $p$ values are shown in the bracket. $A_{12}>0.5$ means the Pareto search is better (highlighted in \colorbox{steel!10}{blue}); $A_{12}<0.5$ denotes the weighted search is better (highlighted in \colorbox{pink!120}{pink}); $A_{12}=0.5$ means a tie. In particular, $0.6\leq A_{12}<0.7$ or $0.3< A_{12}\leq0.4$ indicates a small effect size while $0.7 \leq A_{12} < 0.8$ or $0.2 < A_{12} \leq 0.3$ means a medium effect size; $A_{12} \geq 0.8$ or $0.2 \leq A_{12}$ indicates a large effect size. The comparisons, for which there is a statistically significant differences ($p<$.05) and non-trivial effect size ($A_{12} \leq 0.4$ or $A_{12} \geq 0.6$), are highlighted in \textbf{bold}.
    %\end{tablenotes}
\end{table}

==> tables/quality-abstract.tex <==
\begin{table}[t!]%change two red to two green
\caption{$A_{12}$ values and statistical significance of the comparisons on weighted fitness under identical search budget over 100 runs. A row shows the result over 9 different weight vectors. 6(1):2(0) means that the Pareto search wins 6 cases with $\hat{A}_{12}>0.5$ (1 of them with $\hat{A}_{12}\geq 0.6$ and $p<0.05$), while the weighted search wins on 2 cases with $\hat{A}_{12}<0.5$ (none of which has $\hat{A}_{12}\leq 0.4$ and $p<0.05$); the remaining 1 case is a tie, i.e., $\hat{A}_{12}=0.5$. The comparisons where the Pareto search and its weighed counterpart wins more are shown in \setlength{\fboxsep}{1.5pt}\colorbox{steel!10}{blue} and \setlength{\fboxsep}{1.5pt}\colorbox{red!30}{red}, respectively. Among these, the strategy with more statistically significant wins is shown in bold.}
\label{tb:quality}
\setlength{\tabcolsep}{1.3mm}
\centering
\footnotesize
\begin{tabular}{ccc|cc}\toprule

&\multicolumn{2}{c|}{\textbf{\# Evaluation Budget}}&\multicolumn{2}{c}{\textbf{Time Budget}}\\ \midrule

&\textbf{Rank}&\textbf{Gain Percentile}&\textbf{Rank}&\textbf{Gain Percentile}\\ \midrule




\textsc{wc-c1-3d}&\cellcolor{steel!10}\textbf{9(4)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-wc-c1-3d-eval.pdf}}&\cellcolor{steel!10}\textbf{9(4)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-wc-c1-3d-time.pdf}}\\ 

\textsc{wc-c3-3d}&\cellcolor{steel!10}\textbf{7(6)}:2(2)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-wc-c3-3d-eval.pdf}}&\cellcolor{steel!10}\textbf{7(6)}:2(2)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-wc-c3-3d-time.pdf}}\\ 

\textsc{wc-c4-3d}&\cellcolor{red!30}2(2):\textbf{7(5)}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-wc-c4-3d-eval.pdf}}&\cellcolor{red!30}2(2):\textbf{7(5)}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-wc-c4-3d-time.pdf}}\\ 

\textsc{wc-c5-5d}&0(0):0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-wc-c5-5d-eval.pdf}}&0(0):0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-wc-c5-5d-time.pdf}}\\ 

\textsc{rs-c3-6d}&\cellcolor{steel!10}\textbf{6(6)}:3(2)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-rs-c3-6d-eval.pdf}}&\cellcolor{steel!10}\textbf{6(6)}:3(2)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-rs-c3-6d-time.pdf}}\\ 

\textsc{wc-c1-6d}&\cellcolor{steel!10}\textbf{9(8)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-wc-c1-6d-eval.pdf}}&\cellcolor{steel!10}\textbf{9(8)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-wc-c1-6d-time.pdf}}\\ 

\textsc{llvm}&\cellcolor{steel!10}\textbf{6(1)}:2(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-llvm-eval.pdf}}&\cellcolor{steel!10}\textbf{6(1)}:2(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-llvm-time.pdf}}\\ 

\textsc{trimesh}&\cellcolor{steel!10}\textbf{9(9)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-trimesh-eval.pdf}}&\cellcolor{steel!10}\textbf{9(9)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-trimesh-time.pdf}}\\ 




\textsc{5as-1}&\cellcolor{steel!10}\textbf{8(8)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-5as-1-eval.pdf}}&\cellcolor{steel!10}\textbf{8(8)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-5as-1-time.pdf}}\\ 

\textsc{5as-2}&\cellcolor{steel!10}\textbf{6(6)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-5as-2-eval.pdf}}&\cellcolor{steel!10}\textbf{6(6)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-5as-2-time.pdf}}\\ 

\textsc{5as-3}&\cellcolor{steel!10}\textbf{5(5)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-5as-3-eval.pdf}}&\cellcolor{steel!10}\textbf{5(5)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-5as-3-time.pdf}}\\ 

\textsc{10as-1}&\cellcolor{steel!10}\textbf{8(8)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-10as-1-eval.pdf}}&\cellcolor{steel!10}\textbf{8(8)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-10as-1-time.pdf}}\\ 

\textsc{10as-2}&\cellcolor{steel!10}\textbf{6(5)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-10as-2-eval.pdf}}&\cellcolor{steel!10}\textbf{6(5)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-10as-2-time.pdf}}\\ 

\textsc{10as-3}&\cellcolor{steel!10}\textbf{8(8)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-10as-3-eval.pdf}}&\cellcolor{steel!10}\textbf{8(8)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-10as-3-time.pdf}}\\ 

\textsc{15as-1}&\cellcolor{steel!10}\textbf{8(8)}:1(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-15as-1-eval.pdf}}&\cellcolor{steel!10}\textbf{8(8)}:1(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-15as-1-time.pdf}}\\ 

\textsc{15as-2}&4(0):4(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-15as-2-eval.pdf}}&0(0):9(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-15as-2-time.pdf}}\\ 

\textsc{15as-3}&\cellcolor{steel!10}\textbf{6(3)}:3(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-15as-3-eval.pdf}}&\cellcolor{steel!10}\textbf{3(3)}:6(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-15as-3-time.pdf}}\\ 

\textsc{50as}&\cellcolor{steel!10}\textbf{7(7)}:2(2)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-50as-eval.pdf}}&\cellcolor{red!30}4(3):\textbf{5(5)}&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-50as-time.pdf}}\\ 




\textsc{nrp-e1}&\cellcolor{steel!10}\textbf{8(7)}:1(1)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-e1-eval.pdf}}&\cellcolor{steel!10}\textbf{8(7)}:1(1)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-e1-time.pdf}}\\ 

\textsc{nrp-e2}&\cellcolor{steel!10}\textbf{8(8)}:1(1)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-e2-eval.pdf}}&\cellcolor{steel!10}\textbf{8(8)}:1(1)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-e2-time.pdf}}\\ 

\textsc{nrp-e3}&\cellcolor{steel!10}\textbf{9(9)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-e3-eval.pdf}}&\cellcolor{steel!10}\textbf{9(9)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-e3-time.pdf}}\\ 

\textsc{nrp-e4}&\cellcolor{steel!10}\textbf{8(7)}:1(1)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-e4-eval.pdf}}&\cellcolor{steel!10}\textbf{8(7)}:1(1)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-e4-time.pdf}}\\ 

\textsc{nrp-g1}&\cellcolor{steel!10}\textbf{9(9)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-g1-eval.pdf}}&\cellcolor{steel!10}\textbf{9(9)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-g1-time.pdf}}\\ 

\textsc{nrp-g2}&\cellcolor{steel!10}\textbf{9(9)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-g2-eval.pdf}}&\cellcolor{steel!10}\textbf{9(9)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-g2-time.pdf}}\\ 

\textsc{nrp-g3}&\cellcolor{steel!10}\textbf{8(8)}:1(1)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-g3-eval.pdf}}&\cellcolor{steel!10}\textbf{8(8)}:1(1)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-g3-time.pdf}}\\ 

\textsc{nrp-g4}&\cellcolor{steel!10}\textbf{6(6)}:3(3)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-g4-eval.pdf}}&\cellcolor{steel!10}\textbf{6(6)}:3(3)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-g4-time.pdf}}\\ 

\textsc{nrp-m1}&\cellcolor{steel!10}\textbf{9(8)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-m1-eval.pdf}}&\cellcolor{steel!10}\textbf{9(8)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-m1-time.pdf}}\\ 

\textsc{nrp-m2}&\cellcolor{steel!10}\textbf{9(9)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-m2-eval.pdf}}&\cellcolor{steel!10}\textbf{9(9)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-m2-time.pdf}}\\ 

\textsc{nrp-m3}&\cellcolor{steel!10}\textbf{9(9)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-m3-eval.pdf}}&\cellcolor{steel!10}\textbf{9(9)}:0(0)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-m3-time.pdf}}\\ 

\textsc{nrp-m4}&\cellcolor{steel!10}\textbf{8(8)}:1(1)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-m4-eval.pdf}}&\cellcolor{steel!10}\textbf{8(8)}:1(1)&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/figs/pdf/quality-error-bar-nrp-m4-time.pdf}}\\ 



&&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/quality-error-bar-bottom.pdf}}&&\parbox[c]{0.8in}{\includegraphics[width=0.8in]{tables/embedding/quality-error-bar-bottom.pdf}}\\



%%%%




%%%%


\bottomrule
\end{tabular}




%}
\centering
% \begin{tablenotes}
   % \footnotesize
   % \item The $p$ values are shown in the bracket. $A_{12}>0.5$ means the Pareto search is better (highlighted in \colorbox{steel!10}{blue}); $A_{12}<0.5$ denotes the weighted search is better (highlighted in \colorbox{pink!120}{pink}); $A_{12}=0.5$ means a tie. In particular, $0.6\leq A_{12}<0.7$ or $0.3< A_{12}\leq0.4$ indicates a small effect size while $0.7 \leq A_{12} < 0.8$ or $0.2 < A_{12} \leq 0.3$ means a medium effect size; $A_{12} \geq 0.8$ or $0.2 \leq A_{12}$ indicates a large effect size. The comparisons, for which there is a statistically significant differences ($p<$.05) and non-trivial effect size ($A_{12} \leq 0.4$ or $A_{12} \geq 0.6$), are highlighted in \textbf{bold}.
    %\end{tablenotes}
\end{table}

==> tables/quality-bk.tex <==
\begin{table*}%change two red to two green
\caption{$A_{12}$ values and statistical significance of the comparisons under identical search budget over 100 runs}
\label{tb:quality}
\setlength{\tabcolsep}{1.2mm}
\centering
\footnotesize
\begin{tabular}{ccccccccccc}\toprule

\multirow{2}{*}{\textbf{Problem}}&\multirow{2}{*}{\textbf{Budget}}&\multicolumn{9}{c}{\textbf{Weight Vector}}\\
\cmidrule{3-11}
&&\textbf{[0.1, 0.9]}&\textbf{[0.2, 0.8]}&\textbf{[0.3, 0.7]}&\textbf{[0.4, 0.6]}&\textbf{[0.5, 0.5]}&\textbf{[0.6, 0.4]}&\textbf{[0.7, 0.3]}&\textbf{[0.8, 0.2]}&\textbf{[0.9, 0.1]}\\ 
\midrule

\multirow{2}{*}{\textsc{wc-c1-3d}}&\textbf{\# Evaluations}&\cellcolor{steel!20}.53 ($<$.001)&\cellcolor{green!50}.56 ($<$.001)&\cellcolor{green!50}.62 ($=$.360)&\cellcolor{green!50}\bfseries.85 ($<$.001)&\cellcolor{green!50}\bfseries.82 ($<$.001)&\cellcolor{green!50}\bfseries.74 ($<$.001)&\cellcolor{green!50}\bfseries.74 ($<$.001)&\cellcolor{green!50}\bfseries.80 ($<$.001)&\cellcolor{green!50}\bfseries.75 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}.53 ($<$.001)&\cellcolor{green!50}.56 ($<$.001)&\cellcolor{green!50}.62 ($=$.360)&\cellcolor{green!50}\bfseries.85 ($<$.001)&\cellcolor{green!50}\bfseries.82 ($<$.001)&\cellcolor{green!50}\bfseries.74 ($<$.001)&\cellcolor{green!50}\bfseries.74 ($<$.001)&\cellcolor{green!50}\bfseries.80 ($<$.001)&\cellcolor{green!50}\bfseries.75 ($<$.001)\\

\multirow{2}{*}{\textsc{wc-c3-3d}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries.71 ($<$.001)&\cellcolor{green!50}\bfseries.70 ($<$.001)&\cellcolor{green!50}\bfseries.74 ($<$.001)&\cellcolor{green!50}\bfseries.69 ($<$.001)&\cellcolor{green!50}\bfseries.68 ($<$.001)&\cellcolor{green!50}\bfseries.72 ($<$.001)&\cellcolor{green!50}\bfseries.68 ($<$.001)&\cellcolor{green!50}\bfseries.61 ($=$.008)&\cellcolor{green!50}.59 ($<$.048)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries.71 ($<$.001)&\cellcolor{green!50}\bfseries.70 ($<$.001)&\cellcolor{green!50}\bfseries.74 ($<$.001)&\cellcolor{green!50}\bfseries.69 ($<$.001)&\cellcolor{green!50}\bfseries.68 ($<$.001)&\cellcolor{green!50}\bfseries.72 ($<$.001)&\cellcolor{green!50}\bfseries.68 ($<$.001)&\cellcolor{green!50}\bfseries.61 ($=$.008)&\cellcolor{green!50}.59 ($<$.048)\\

\multirow{2}{*}{\textsc{wc-c4-3d}}&\textbf{\# Evaluations}&\cellcolor{red!50}.47 ($=$.674)&\cellcolor{red!50}.49 ($=$.549)&\cellcolor{green!50}.58 ($=$.128)&\cellcolor{green!50}.55 ($=$.186)&\cellcolor{red!50}.40 ($=$.030)&\cellcolor{red!50}\bfseries.33 ($<$.001)&\cellcolor{red!50}.41 ($=$.158)&\cellcolor{green!50}.52 ($=$.045)&\cellcolor{red!50}.42 ($=$.249)\\
&\textbf{Time}&\cellcolor{red!50}.47 ($=$.674)&\cellcolor{red!50}.49 ($=$.549)&\cellcolor{green!50}.58 ($=$.128)&\cellcolor{green!50}.55 ($=$.186)&\cellcolor{red!50}.40 ($=$.030)&\cellcolor{red!50}\bfseries.33 ($<$.001)&\cellcolor{red!50}.41 ($=$.158)&\cellcolor{green!50}.52 ($=$.045)&\cellcolor{red!50}.42 ($=$.249)\\

\multirow{2}{*}{\textsc{wc-c5-5d}}&\textbf{\# Evaluations}&\cellcolor{green!50}.52 ($=$.922)&\cellcolor{green!50}.57 ($=$.639)&\cellcolor{green!50}.53 ($=$.490)&\cellcolor{red!50}.49 ($=$.017)&\cellcolor{red!50}.49 ($=$.010)&\cellcolor{green!50}.51 ($=$.012)&\cellcolor{green!50}.55 ($=$.765)&\cellcolor{green!50}.55 ($=$.487)&\cellcolor{green!50}.54 ($=$.281)\\
&\textbf{Time}&\cellcolor{green!50}.52 ($=$.922)&\cellcolor{green!50}.57 ($=$.639)&\cellcolor{green!50}.53 ($=$.490)&\cellcolor{pink}.49 ($=$.017)&\cellcolor{red!50}.49 ($=$.010)&\cellcolor{green!50}.51 ($=$.012)&\cellcolor{green!50}.55 ($=$.765)&\cellcolor{green!50}.55 ($=$.487)&\cellcolor{green!50}.54 ($=$.281)\\

\multirow{2}{*}{\textsc{rs-c3-6d}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries.96 ($<$.001)&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries.87 ($<$.001)&\cellcolor{green!50}\bfseries.92 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.68 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries.96 ($<$.001)&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries.87 ($<$.001)&\cellcolor{green!50}\bfseries.92 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.68 ($<$.001)\\

\multirow{2}{*}{\textsc{wc-c1-6d}}&\textbf{\# Evaluations}&.50 ($=$.798)&\cellcolor{red!50}.45 ($=$.031)&\cellcolor{red!50}.47 ($=$.033)&\cellcolor{red!50}.42 ($<$.001)&\cellcolor{green!50}.52 ($=$.396)&\cellcolor{green!50}\bfseries.76 ($<$.001)&\cellcolor{red!50}.48 ($=$.004)&\cellcolor{red!50}.43 ($<$.001)&\cellcolor{green!50}\bfseries.65 ($<$.001)\\
&\textbf{Time}&.50 ($=$.798)&\cellcolor{red!50}.45 ($=$.031)&\cellcolor{red!50}.47 ($=$.033)&\cellcolor{red!50}.42 ($<$.001)&\cellcolor{green!50}.52 ($=$.396)&\cellcolor{green!50}\bfseries.76 ($<$.001)&\cellcolor{red!50}.48 ($=$.004)&\cellcolor{red!50}.43 ($<$.001)&\cellcolor{green!50}\bfseries.65 ($<$.001)\\

\multirow{2}{*}{\textsc{llvm}}&\textbf{\# Evaluations}&\cellcolor{green!50}.56 ($<$.001)&.50 ($=$.999)&\cellcolor{green!50}.53 ($<$.001)&\cellcolor{green!50}.59 ($=$.116)&\cellcolor{green!50}.56 ($=$.001)&\cellcolor{green!50}.57 ($<$.002)&\cellcolor{green!50}.63 ($=$.959)&\cellcolor{green!50}.66 ($<$.128)&\cellcolor{red!50}.47 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}.56 ($<$.001)&.50 ($=$.999)&\cellcolor{green!50}.53 ($<$.001)&\cellcolor{green!50}.59 ($=$.116)&\cellcolor{green!50}.56 ($=$.001)&\cellcolor{green!50}.57 ($<$.002)&\cellcolor{green!50}.63 ($=$.959)&\cellcolor{green!50}.66 ($<$.128)&\cellcolor{red!50}.47 ($<$.001)\\

\multirow{2}{*}{\textsc{trimesh}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

%%%%%%%%%%%

\multirow{2}{*}{\textsc{5as-1}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{5as-2}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&.50 ($=$.999)&.50 ($=$.999)&.50 ($=$.999)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&.50 ($=$.999)&.50 ($=$.999)&.50 ($=$.999)\\

\multirow{2}{*}{\textsc{5as-3}}&\textbf{\# Evaluations}&.50 ($=$.999)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&.50 ($=$.999)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\


\multirow{2}{*}{\textsc{10as-1}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{10as-2}}&\textbf{\# Evaluations}&\cellcolor{green!50}.53 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}.54 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{10as-3}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{15as-1}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{15as-2}}&\textbf{\# Evaluations}&\cellcolor{red!50}.49 ($<$.001)&\cellcolor{red!50}.49 ($<$.001)&\cellcolor{red!50}.49 ($<$.001)&\cellcolor{red!50}.48 ($<$.001)&\cellcolor{green!50}.51 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{red!50}.48 ($<$.001)&\cellcolor{red!50}.48 ($<$.001)&\cellcolor{red!50}.48 ($<$.001)&\cellcolor{red!50}.48 ($<$.001)&\cellcolor{red!50}.48 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{15as-3}}&\textbf{\# Evaluations}&\cellcolor{red!50}.48 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.86 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}.51 ($<$.001)&\cellcolor{red!50}.49 ($<$.001)&\cellcolor{red!50}.49 ($<$.001)\\
&\textbf{Time}&\cellcolor{red!50}.46 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.87 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{red!50}.46 ($<$.001)&\cellcolor{red!50}.46 ($<$.001)&\cellcolor{red!50}.46 ($<$.001)\\

\multirow{2}{*}{\textsc{50as}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries.93 ($<$.001)&\cellcolor{green!50}\bfseries.97 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries.90 ($<$.001)&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

%%%%%%%%%%%

\multirow{2}{*}{\textsc{nrp-e1}}&\textbf{\# Evaluations}&\cellcolor{red!50}\bfseries.02 ($<$.001)&\cellcolor{green!50}\bfseries.95 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{red!50}\bfseries.02 ($<$.001)&\cellcolor{green!50}\bfseries.94 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-e2}}&\textbf{\# Evaluations}&\cellcolor{red!50}\bfseries.04 ($<$.001)&\cellcolor{green!50}\bfseries.94 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{red!50}\bfseries.04 ($<$.001)&\cellcolor{green!50}\bfseries.94 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-e3}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries.89 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.88 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-e4}}&\textbf{\# Evaluations}&\cellcolor{red!50}\bfseries.03 ($<$.001)&\cellcolor{green!50}\bfseries.96 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{red!50}\bfseries.04 ($<$.001)&\cellcolor{green!50}\bfseries.96 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-g1}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries.86 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries.74 ($<$.001)&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-g2}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries.85 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries.80 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-g3}}&\textbf{\# Evaluations}&\cellcolor{red!50}\bfseries.08 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{red!50}\bfseries.08 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-g4}}&\textbf{\# Evaluations}&\cellcolor{red!50}\bfseries.34 ($<$.001)&\cellcolor{red!50}\bfseries.22 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.92 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{red!50}\bfseries.33 ($<$.001)&\cellcolor{red!50}\bfseries.19 ($<$.001)&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries.93 ($<$.001)&\cellcolor{green!50}\bfseries.97 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-m1}}&\textbf{\# Evaluations}&\cellcolor{green!50}.47 ($=$.036)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}.42 ($=$.036)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-m2}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries.76 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries.72 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-m3}}&\textbf{\# Evaluations}&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-m4}}&\textbf{\# Evaluations}&\cellcolor{red!50}\bfseries.33 ($<$.001)&\cellcolor{green!50}\bfseries.67 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries.95 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)\\
&\textbf{Time}&\cellcolor{red!50}\bfseries.37 ($<$.001)&\cellcolor{green!50}\bfseries.61 ($=$.003)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries.90 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)\\

\bottomrule
\end{tabular}
%}
\centering
 \begin{tablenotes}
    \footnotesize
    \item The $p$ values are shown in the bracket. $A_{12}>0.5$ means the Pareto search is better (highlighted in \colorbox{green!50}{green}); $A_{12}<0.5$ denotes the weighted search is better (highlighted in \colorbox{red!50}{red}); $A_{12}=0.5$ means a tie. In particular, $0.6\leq A_{12}<0.7$ or $0.3< A_{12}\leq0.4$ indicates a small effect size while $0.7 \leq A_{12} < 0.8$ or $0.2 < A_{12} \leq 0.3$ means a medium effect size; $A_{12} \geq 0.8$ or $0.2 \leq A_{12}$ indicates a large effect size. The comparisons, for which there is a statistically significant differences ($p<$.05) and non-trivial effect size ($A_{12} \leq 0.4$ or $A_{12} \geq 0.6$), are highlighted in \textbf{bold}.
    \end{tablenotes}
\end{table*}

==> tables/quality.tex <==
\begin{table*}%change two red to two green
\caption{$A_{12}$ values and statistical significance of the comparisons on weighted fitness under identical search budget over 100 runs.}
\label{tb:quality}
\setlength{\tabcolsep}{1.2mm}
\centering
\footnotesize
\begin{tabular}{ccccccccccc}\toprule

\multirow{2}{*}[-0.1cm]{\textbf{\makecell{SBSE\\Problem}}}&\multirow{2}{*}[-0.08cm]{\textbf{\makecell{Budget\\Type}}}&\multicolumn{9}{c}{\textbf{Weight Vector}}\\
\cmidrule{3-11}
&&$\mathbf{(0.1,0.9)}$&$\mathbf{(0.2,0.8)}$&$\mathbf{(0.3,0.7)}$&$\mathbf{(0.4,0.6)}$&$\mathbf{(0.5,0.5)}$&$\mathbf{(0.6,0.4)}$&$\mathbf{(0.7,0.3)}$&$\mathbf{(0.8,0.2)}$&$\mathbf{(0.9,0.1)}$\\ 
\midrule

\multirow{2}{*}{\textsc{wc-c1-3d}}&\textbf{\# Evaluations}&\cellcolor{steel!10}.53 ($<$.001)&\cellcolor{steel!10}.56 ($<$.001)&\cellcolor{steel!10}.62 ($=$.360)&\cellcolor{steel!10}\bfseries.85 ($<$.001)&\cellcolor{steel!10}\bfseries.82 ($<$.001)&\cellcolor{steel!10}\bfseries.74 ($<$.001)&\cellcolor{steel!10}\bfseries.74 ($<$.001)&\cellcolor{steel!10}\bfseries.80 ($<$.001)&\cellcolor{steel!10}\bfseries.75 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}.53 ($<$.001)&\cellcolor{steel!10}.56 ($<$.001)&\cellcolor{steel!10}.62 ($=$.360)&\cellcolor{steel!10}\bfseries.85 ($<$.001)&\cellcolor{steel!10}\bfseries.82 ($<$.001)&\cellcolor{steel!10}\bfseries.74 ($<$.001)&\cellcolor{steel!10}\bfseries.74 ($<$.001)&\cellcolor{steel!10}\bfseries.80 ($<$.001)&\cellcolor{steel!10}\bfseries.75 ($<$.001)\\

\multirow{2}{*}{\textsc{wc-c3-3d}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries.71 ($<$.001)&\cellcolor{steel!10}\bfseries.70 ($<$.001)&\cellcolor{steel!10}\bfseries.74 ($<$.001)&\cellcolor{steel!10}\bfseries.69 ($<$.001)&\cellcolor{steel!10}\bfseries.68 ($<$.001)&\cellcolor{steel!10}\bfseries.72 ($<$.001)&\cellcolor{steel!10}\bfseries.68 ($<$.001)&\cellcolor{steel!10}\bfseries.61 ($=$.008)&\cellcolor{steel!10}.59 ($=$.048)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries.71 ($<$.001)&\cellcolor{steel!10}\bfseries.70 ($<$.001)&\cellcolor{steel!10}\bfseries.74 ($<$.001)&\cellcolor{steel!10}\bfseries.69 ($<$.001)&\cellcolor{steel!10}\bfseries.68 ($<$.001)&\cellcolor{steel!10}\bfseries.72 ($<$.001)&\cellcolor{steel!10}\bfseries.68 ($<$.001)&\cellcolor{steel!10}\bfseries.61 ($=$.008)&\cellcolor{steel!10}.59 ($=$.048)\\

\multirow{2}{*}{\textsc{wc-c4-3d}}&\textbf{\# Evaluations}&\cellcolor{pink!120}.47 ($=$.674)&\cellcolor{pink!120}.49 ($=$.549)&\cellcolor{steel!10}.58 ($=$.128)&\cellcolor{steel!10}.55 ($=$.186)&\cellcolor{pink!120}.40 ($=$.030)&\cellcolor{pink!120}\bfseries.33 ($<$.001)&\cellcolor{pink!120}.41 ($=$.158)&\cellcolor{steel!10}.52 ($=$.045)&\cellcolor{pink!120}.42 ($=$.249)\\
&\textbf{Time}&\cellcolor{pink!120}.47 ($=$.674)&\cellcolor{pink!120}.49 ($=$.549)&\cellcolor{steel!10}.58 ($=$.128)&\cellcolor{steel!10}.55 ($=$.186)&\cellcolor{pink!120}.40 ($=$.030)&\cellcolor{pink!120}\bfseries.33 ($<$.001)&\cellcolor{pink!120}.41 ($=$.158)&\cellcolor{steel!10}.52 ($=$.045)&\cellcolor{pink!120}.42 ($=$.249)\\

\multirow{2}{*}{\textsc{wc-c5-5d}}&\textbf{\# Evaluations}&\cellcolor{steel!10}.52 ($=$.922)&\cellcolor{steel!10}.57 ($=$.639)&\cellcolor{steel!10}.53 ($=$.490)&\cellcolor{pink!120}.49 ($=$.017)&\cellcolor{pink!120}.49 ($=$.010)&\cellcolor{steel!10}.51 ($=$.012)&\cellcolor{steel!10}.55 ($=$.765)&\cellcolor{steel!10}.55 ($=$.487)&\cellcolor{steel!10}.54 ($=$.281)\\
&\textbf{Time}&\cellcolor{steel!10}.52 ($=$.922)&\cellcolor{steel!10}.57 ($=$.639)&\cellcolor{steel!10}.53 ($=$.490)&\cellcolor{pink!120}.49 ($=$.017)&\cellcolor{pink!120}.49 ($=$.010)&\cellcolor{steel!10}.51 ($=$.012)&\cellcolor{steel!10}.55 ($=$.765)&\cellcolor{steel!10}.55 ($=$.487)&\cellcolor{steel!10}.54 ($=$.281)\\

\multirow{2}{*}{\textsc{rs-c3-6d}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries.96 ($<$.001)&\cellcolor{steel!10}\bfseries.98 ($<$.001)&\cellcolor{steel!10}\bfseries.87 ($<$.001)&\cellcolor{steel!10}\bfseries.92 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries.68 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries.96 ($<$.001)&\cellcolor{steel!10}\bfseries.98 ($<$.001)&\cellcolor{steel!10}\bfseries.87 ($<$.001)&\cellcolor{steel!10}\bfseries.92 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries.68 ($<$.001)\\

\multirow{2}{*}{\textsc{wc-c1-6d}}&\textbf{\# Evaluations}&.50 ($=$.798)&\cellcolor{pink!120}.45 ($=$.031)&\cellcolor{pink!120}.47 ($=$.033)&\cellcolor{pink!120}.42 ($<$.001)&\cellcolor{steel!10}.52 ($=$.396)&\cellcolor{steel!10}\bfseries.76 ($<$.001)&\cellcolor{pink!120}.48 ($=$.004)&\cellcolor{pink!120}.43 ($<$.001)&\cellcolor{steel!10}\bfseries.65 ($<$.001)\\
&\textbf{Time}&.50 ($=$.798)&\cellcolor{pink!120}.45 ($=$.031)&\cellcolor{pink!120}.47 ($=$.033)&\cellcolor{pink!120}.42 ($<$.001)&\cellcolor{steel!10}.52 ($=$.396)&\cellcolor{steel!10}\bfseries.76 ($<$.001)&\cellcolor{pink!120}.48 ($=$.004)&\cellcolor{pink!120}.43 ($<$.001)&\cellcolor{steel!10}\bfseries.65 ($<$.001)\\

\multirow{2}{*}{\textsc{llvm}}&\textbf{\# Evaluations}&\cellcolor{steel!10}.56 ($<$.001)&.50 ($=$.999)&\cellcolor{steel!10}.53 ($<$.001)&\cellcolor{steel!10}.59 ($=$.116)&\cellcolor{steel!10}.56 ($=$.001)&\cellcolor{steel!10}.57 ($<$.002)&\cellcolor{steel!10}.63 ($=$.959)&\cellcolor{steel!10}.66 ($=$.128)&\cellcolor{pink!120}.47 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}.56 ($<$.001)&.50 ($=$.999)&\cellcolor{steel!10}.53 ($<$.001)&\cellcolor{steel!10}.59 ($=$.116)&\cellcolor{steel!10}.56 ($=$.001)&\cellcolor{steel!10}.57 ($<$.002)&\cellcolor{steel!10}.63 ($=$.959)&\cellcolor{steel!10}.66 ($=$.128)&\cellcolor{pink!120}.47 ($<$.001)\\

\multirow{2}{*}{\textsc{trimesh}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries.98 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries.98 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

%%%%%%%%%%%

\multirow{2}{*}{\textsc{5as-1}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{5as-2}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&.50 ($=$.999)&.50 ($=$.999)&.50 ($=$.999)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&.50 ($=$.999)&.50 ($=$.999)&.50 ($=$.999)\\

\multirow{2}{*}{\textsc{5as-3}}&\textbf{\# Evaluations}&.50 ($=$.999)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&.50 ($=$.999)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\


\multirow{2}{*}{\textsc{10as-1}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{10as-2}}&\textbf{\# Evaluations}&\cellcolor{steel!10}.53 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}.54 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{10as-3}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{15as-1}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{15as-2}}&\textbf{\# Evaluations}&\cellcolor{pink!120}.49 ($<$.001)&\cellcolor{pink!120}.49 ($<$.001)&\cellcolor{pink!120}.49 ($<$.001)&\cellcolor{pink!120}.48 ($<$.001)&\cellcolor{steel!10}.51 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{pink!120}.48 ($<$.001)&\cellcolor{pink!120}.48 ($<$.001)&\cellcolor{pink!120}.48 ($<$.001)&\cellcolor{pink!120}.48 ($<$.001)&\cellcolor{pink!120}.48 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{15as-3}}&\textbf{\# Evaluations}&\cellcolor{pink!120}.48 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries.86 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}.51 ($<$.001)&\cellcolor{pink!120}.49 ($<$.001)&\cellcolor{pink!120}.49 ($<$.001)\\
&\textbf{Time}&\cellcolor{pink!120}.46 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries.87 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{pink!120}.46 ($<$.001)&\cellcolor{pink!120}.46 ($<$.001)&\cellcolor{pink!120}.46 ($<$.001)\\

\multirow{2}{*}{\textsc{50as}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries.93 ($<$.001)&\cellcolor{steel!10}\bfseries.97 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries.90 ($<$.001)&\cellcolor{steel!10}\bfseries.98 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

%%%%%%%%%%%

\multirow{2}{*}{\textsc{nrp-e1}}&\textbf{\# Evaluations}&\cellcolor{pink!120}\bfseries.02 ($<$.001)&\cellcolor{steel!10}\bfseries.95 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{pink!120}\bfseries.02 ($<$.001)&\cellcolor{steel!10}\bfseries.94 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-e2}}&\textbf{\# Evaluations}&\cellcolor{pink!120}\bfseries.04 ($<$.001)&\cellcolor{steel!10}\bfseries.94 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{pink!120}\bfseries.04 ($<$.001)&\cellcolor{steel!10}\bfseries.94 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-e3}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries.89 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries.88 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-e4}}&\textbf{\# Evaluations}&\cellcolor{pink!120}\bfseries.03 ($<$.001)&\cellcolor{steel!10}\bfseries.96 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{pink!120}\bfseries.04 ($<$.001)&\cellcolor{steel!10}\bfseries.96 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-g1}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries.86 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries.74 ($<$.001)&\cellcolor{steel!10}\bfseries.98 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-g2}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries.85 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries.80 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-g3}}&\textbf{\# Evaluations}&\cellcolor{pink!120}\bfseries.08 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{pink!120}\bfseries.08 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-g4}}&\textbf{\# Evaluations}&\cellcolor{pink!120}\bfseries.34 ($<$.001)&\cellcolor{pink!120}\bfseries.22 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries.92 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{pink!120}\bfseries.33 ($<$.001)&\cellcolor{pink!120}\bfseries.19 ($<$.001)&\cellcolor{steel!10}\bfseries.98 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries.93 ($<$.001)&\cellcolor{steel!10}\bfseries.97 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-m1}}&\textbf{\# Evaluations}&\cellcolor{pink!120}.47 ($=$.036)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{pink!120}.42 ($=$.036)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-m2}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries.76 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries.72 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-m3}}&\textbf{\# Evaluations}&\cellcolor{steel!10}\bfseries.98 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\
&\textbf{Time}&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries.98 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)\\

\multirow{2}{*}{\textsc{nrp-m4}}&\textbf{\# Evaluations}&\cellcolor{pink!120}\bfseries.33 ($<$.001)&\cellcolor{steel!10}\bfseries.67 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries.95 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)\\
&\textbf{Time}&\cellcolor{pink!120}\bfseries.37 ($<$.001)&\cellcolor{steel!10}\bfseries.61 ($=$.003)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries1.0 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)&\cellcolor{steel!10}\bfseries.90 ($<$.001)&\cellcolor{steel!10}\bfseries.99 ($<$.001)\\

\bottomrule
\end{tabular}
%}
\centering
 \begin{tablenotes}
    \footnotesize
    \item The $p$ values are shown in the bracket. $A_{12}>0.5$ means the Pareto search is better (highlighted in \colorbox{steel!10}{blue}); $A_{12}<0.5$ denotes the weighted search is better (highlighted in \colorbox{pink!120}{pink}); $A_{12}=0.5$ means a tie. In particular, $0.6\leq A_{12}<0.7$ or $0.3< A_{12}\leq0.4$ indicates a small effect size while $0.7 \leq A_{12} < 0.8$ or $0.2 < A_{12} \leq 0.3$ means a medium effect size; $A_{12} \geq 0.8$ or $0.2 \leq A_{12}$ indicates a large effect size. The comparisons, for which there is a statistically significant differences ($p<$.05) and non-trivial effect size ($A_{12} \leq 0.4$ or $A_{12} \geq 0.6$), are highlighted in \textbf{bold}.
    \end{tablenotes}
\end{table*}

==> tables/quality_time.tex <==
\begin{table*}
\caption{$A_{12}$ values and statistical significance of the comparisons under the same number of evaluations over all 100 runs}
\label{tb:quality}
%\setlength{\tabcolsep}{7mm}{
\centering
\begin{tabular}{cccccccccc}\toprule

\multirow{2}{*}{\textbf{Problem}}&\multicolumn{9}{c}{\textbf{Weight Vector}}\\
\cmidrule{2-10}
&\textbf{[0.1, 0.9]}&\textbf{[0.2, 0.8]}&\textbf{[0.3, 0.7]}&\textbf{[0.4, 0.6]}&\textbf{[0.5, 0.5]}&\textbf{[0.6, 0.4]}&\textbf{[0.7, 0.3]}&\textbf{[0.8, 0.2]}&\textbf{[0.9, 0.1]}\\ 
\midrule

\textsc{wc-c1-3d}&\cellcolor{green!50}.53 ($<$.001)&\cellcolor{green!50}.56 ($<$.001)&\cellcolor{green!50}.62 ($=$.360)&\cellcolor{green!50}\bfseries.85 ($<$.001)&\cellcolor{green!50}\bfseries.82 ($<$.001)&\cellcolor{green!50}\bfseries.74 ($<$.001)&\cellcolor{green!50}\bfseries.74 ($<$.001)&\cellcolor{green!50}\bfseries.80 ($<$.001)&\cellcolor{green!50}\bfseries.75 ($<$.001)\\

\textsc{wc-c3-3d}&\cellcolor{green!50}\bfseries.71 ($<$.001)&\cellcolor{green!50}\bfseries.70 ($<$.001)&\cellcolor{green!50}\bfseries.74 ($<$.001)&\cellcolor{green!50}\bfseries.69 ($<$.001)&\cellcolor{green!50}\bfseries.68 ($<$.001)&\cellcolor{green!50}\bfseries.72 ($<$.001)&\cellcolor{green!50}\bfseries.68 ($<$.001)&\cellcolor{green!50}\bfseries.61 ($=$.008)&\cellcolor{green!50}.59 ($<$.048)\\

\textsc{wc-c4-3d}&\cellcolor{red!50}.47 ($=$.674)&\cellcolor{red!50}.49 ($=$.549)&\cellcolor{green!50}.58 ($=$.128)&\cellcolor{green!50}.55 ($=$.186)&\cellcolor{red!50}.40 ($=$.030)&\cellcolor{red!50}\bfseries.33 ($<$.001)&\cellcolor{red!50}.41 ($=$.158)&\cellcolor{green!50}.52 ($=$.045)&\cellcolor{red!50}.42 ($=$.249)\\

\textsc{wc-c5-5d}&\cellcolor{green!50}.52 ($=$.922)&\cellcolor{green!50}.57 ($=$.639)&\cellcolor{green!50}.53 ($=$.490)&\cellcolor{red!50}.49 ($=$.017)&\cellcolor{red!50}.49 ($=$.010)&\cellcolor{green!50}.51 ($=$.012)&\cellcolor{green!50}.55 ($=$.765)&\cellcolor{green!50}.55 ($=$.487)&\cellcolor{green!50}.54 ($=$.281)\\

\textsc{rs-c3-6d}&\cellcolor{green!50}\bfseries.96 ($<$.001)&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries.87 ($<$.001)&\cellcolor{green!50}\bfseries.92 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.68 ($<$.001)\\

\textsc{wc-c1-6d}&.50 ($=$.798)&\cellcolor{red!50}.45 ($=$.031)&\cellcolor{red!50}.47 ($=$.033)&\cellcolor{red!50}.42 ($<$.001)&\cellcolor{red!50}.52 ($=$.396)&\cellcolor{green!50}\bfseries.76 ($<$.001)&\cellcolor{red!50}.48 ($=$.004)&\cellcolor{red!50}.43 ($<$.001)&\cellcolor{green!50}\bfseries.65 ($<$.001)\\

\textsc{llvm}&\cellcolor{green!50}.56 ($<$.001)&.50 ($=$.999)&\cellcolor{green!50}.53 ($<$.001)&\cellcolor{green!50}.59 ($=$.116)&\cellcolor{green!50}.56 ($=$.001)&\cellcolor{green!50}.57 ($<$.002)&\cellcolor{green!50}.63 ($=$.959)&\cellcolor{green!50}.66 ($<$.128)&\cellcolor{red!50}.47 ($<$.001)\\

\textsc{trimesh}&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

%%%%%%%%%%%

\textsc{5as-1}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{5as-2}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&.50 ($=$.999)&.50 ($=$.999)&.50 ($=$.999)\\

\textsc{5as-3}&.50 ($=$.999)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{10as-1}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{10as-2}&\cellcolor{green!50}.54 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{10as-3}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{15as-1}&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{15as-2}&\cellcolor{red!50}.48 ($<$.001)&\cellcolor{red!50}.48 ($<$.001)&\cellcolor{red!50}.48 ($<$.001)&\cellcolor{red!50}.48 ($<$.001)&\cellcolor{red!50}.48 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{15as-3}&\cellcolor{red!50}.46 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.87 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{red!50}.46 ($<$.001)&\cellcolor{red!50}.46 ($<$.001)&\cellcolor{red!50}.46 ($<$.001)\\

\textsc{50as}&\cellcolor{green!50}\bfseries.96 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

%%%%%%%%%%%

\textsc{nrp-e1}&\cellcolor{red!50}\bfseries.02 ($<$.001)&\cellcolor{green!50}\bfseries.94 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{nrp-e2}&\cellcolor{red!50}\bfseries.04 ($<$.001)&\cellcolor{green!50}\bfseries.94 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{nrp-e3}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.88 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{nrp-e4}&\cellcolor{red!50}\bfseries.04 ($<$.001)&\cellcolor{green!50}\bfseries.96 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{nrp-g1}&\cellcolor{green!50}\bfseries.74 ($<$.001)&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{nrp-g2}&\cellcolor{green!50}\bfseries.80 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{nrp-g3}&\cellcolor{red!50}\bfseries.08 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{nrp-g4}&\cellcolor{red!50}\bfseries.33 ($<$.001)&\cellcolor{red!50}\bfseries.19 ($<$.001)&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries.93 ($<$.001)&\cellcolor{green!50}\bfseries.97 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{nrp-m1}&\cellcolor{green!50}.42 ($=$.036)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{nrp-m2}&\cellcolor{green!50}\bfseries.72 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{nrp-m3}&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.98 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)\\

\textsc{nrp-m4}&\cellcolor{red!50}\bfseries.37 ($<$.001)&\cellcolor{green!50}\bfseries.61 ($=$.003)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries1.0 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)&\cellcolor{green!50}\bfseries.90 ($<$.001)&\cellcolor{green!50}\bfseries.99 ($<$.001)\\




\bottomrule
\end{tabular}
%}
\centering
 \begin{tablenotes}
    \footnotesize
    \item The $p$ values are shown in the bracket. $A_{12}>0.5$ means the Pareto-based search is better (highlighted in \colorbox{green!50}{green}); $A_{12}<0.5$ denotes the weighted search is better (highlighted in \colorbox{red!50}{red}); $A_{12}=0.5$ means a tie. In particular, $0.6\leq A_{12}<0.7$ or $0.3< A_{12}\leq0.4$ indicates a small effect size while $0.7 \leq A_{12} < 0.8$ or $0.2 < A_{12} \leq 0.3$ means a medium effect size; $A_{12} \geq 0.8$ or $0.2 \leq A_{12}$ indicates a large effect size. The comparisons, for which there is a statistically significant differences ($p<$.05) and non-trivial effect size ($A_{12} \leq 0.4$ or $A_{12} \geq 0.6$), are highlighted in \textbf{bold}.
    \end{tablenotes}
\end{table*}

==> tables/settings-bk.tex <==
\begin{table}
\caption{Parameter settings of (some) optimizers.}
\label{tb:settings}
\setlength{\tabcolsep}{1.8mm}
\footnotesize
\centering
\begin{tabular}{cccccc}\toprule

\textbf{Problem/Instance}&$\lvert \mathbfcal{M} \rvert$&$\lvert \mathbfcal{C} \rvert$&$\lvert \mathbfcal{P} \rvert$&$\lvert \mathbfcal{G} \rvert$&$\lvert \mathbfcal{E} \rvert$\\
\midrule

\makecell{\textsc{wc-c1-3d},\textsc{wc-c3-3d}\\\textsc{wc-c5-5d}}&0.1&0.9&20&25&600\\
\rowcolor{steel!10}{\textsc{llvm}}&0.1&0.9&20&25&500\\
\textsc{wc-c4-3d}&0.1&0.9&20&15&300\\
\rowcolor{steel!10}{\textsc{rs-c3-6d},\textsc{wc-c1-6d}}&0.1&0.9&50&30&1.5$\times 10^3$\\
\textsc{trimesh}&0.1&0.9&100&100&$10^4$\\
\hline

\rowcolor{steel!10}\textsc{50as}&0.02&0.8&100&500&5.0$\times 10^4$\\
Other workflows for {WSC}&0.1&0.9&100&300&3.0$\times 10^4$\\

\hline

All projects/versions for {NRP}&0.01&0.8&100&200&2.0$\times 10^4$\\




\bottomrule
\end{tabular}
%}
\centering
 \begin{tablenotes}
    \footnotesize
    \item $\lvert \mathbfcal{M} \rvert$, $\lvert \mathbfcal{C} \rvert$, $\lvert \mathbfcal{P} \rvert$, $\lvert \mathbfcal{G} \rvert$, and $\lvert \mathbfcal{E} \rvert$ denote the mutation rate, crossover rate, population size, \# generations and \# evaluations, respectively.
    \end{tablenotes}
\end{table}
